PowerMove: Optimizing Compilation for Neutral Atom Quantum Computers with Zoned Architecture

Neutral atom-based quantum computers (NAQCs) have recently emerged as promising candidates for scalable quantum computing, largely due to their advanced hardware capabilities, particularly qubit movement and the zoned architecture (ZA). However, fully leveraging these features poses significant compiler challenges, as it requires addressing complexities across gate scheduling, qubit allocation, qubit movement, and inter-zone communication. In this paper, we present PowerMove, an efficient compiler for NAQCs that enhances the qubit movement framework while fully integrating the advantages of ZA. By recognizing and leveraging the interdependencies between these key aspects, PowerMove unlocks new optimization opportunities, significantly enhancing both scalability and fidelity. Our evaluation demonstrates an improvement in fidelity by several orders of magnitude compared to the state-of-the-art methods, with execution time improved by up to 3.46x and compilation time reduced by up to 213.5x. We will open-source our code later to foster further research and collaboration within the community.

==> TexFile/02_Intro_01.tex <==
\section{Introduction}\label{sec:intro}
Quantum computing (QC) is swiftly evolving from a theoretical concept into a tangible reality, with significant advancements across various platforms over the past few decades~\cite{arute2019quantum, huang2020superconducting, bravyi2022future, bruzewicz2019trapped, chen2023benchmarking, kok2007linear, bourassa2021blueprint, bluvstein2024logical, wurtz2023aquila}. Given the rapid progress and the unique strengths of each platform, competition among these platforms is expected to persist for the foreseeable future.

In recent years, \emph{neutral atom-based quantum computers (NAQC)}~\cite{ebadi2021quantum, graham2022multi, wurtz2023aquila, bluvstein2024logical} have emerged as a strong candidate in the QC landscape, owing to their distinct hardware advantages. NAQC systems offer impressive scalability, supporting hundreds~\cite{ebadi2022quantum, wurtz2023aquila, ebadi2021quantum} to $6100$ qubits~\cite{manetsch2024tweezer}, long coherence times of several seconds~\cite{evered2023high, young2020half, barnes2022assembly}, and high-fidelity single-qubit rotations~\cite{bluvstein2024logical, levine2022dispersive, bluvstein2022quantum} as well as two-qubit CZ gates~\cite{levine2019parallel, fu2022high, evered2023high}, achieving fidelities up to $99.99\%$ and $99.5\%$, respectively. A compelling feature of NAQC is the ability to move qubits using \emph{optical traps}~\cite{bluvstein2022quantum}, which enables non-local connectivity and dynamic qubit layout, opening new avenues for enhancing computational efficiency. This culminates in the demonstration of the \emph{zoned architecture (ZA)}~\cite{bluvstein2024logical} that divides the system into distinct zones for specific tasks such as storage and entangling, with qubits shuttled between them--akin to the classical architectures with separate memory and processing units--improving overall system performance.

While promising, fully leveraging these advantages poses considerable challenges due to qubit movement constraints (more details in Sec.\ref{sec:background}). \textbf{First}, qubits can only be moved collectively within a 2D lattice, where the relative order of rows and columns must remain fixed~\cite{bluvstein2022quantum}. This restriction means that desired single-qubit movements usually cannot be executed in one step but must be scheduled over multiple collective movements, increasing total movement time and decoherence error. \textbf{Second}, collective movements often involve \emph{transferring} qubits into the mobile lattice and others into fixed positions. This process introduces both time overhead and the risk of atom loss. \textbf{Third}, movement speed is limited to preserve state coherence, leading to further delays for long-distance moves. Effectively managing all of these constraints is non-trivial but essential for fully utilizing NAQC's qubit movement capabilities.

% Failure to effectively address these constraints can result in significant time overhead, leading to higher decoherence errors that degrade output fidelity.

% , making it crucial to minimize these operations
% As a result, all the desired single qubit movements cannot be performed collectively within a frame, but have to be scheduled across multiple collective movements.

Several compilation frameworks have been developed~\cite{wang2024atomique, wang2023q, tan2022qubit, tan2024compiling, bochen2024compilation} to address the challenges of qubit movement constraints. The approaches in~\cite{wang2024atomique, wang2023q} prohibit qubit transfers by pre-assigning static and mobile qubits, using SWAP gates or ancilla qubits for routing to enable interactions of distant static qubits. While this avoids the risk of atom loss from qubit transfers, the extra SWAP gates significantly reduce fidelity. In contrast, works~\cite{tan2022qubit, tan2024compiling} allow qubit transfers and use solver-based methods to minimize collective movements. Although it avoids additional two-qubit gates, it suffers from scalability issues. The recent compiler \emph{Enola}~\cite{bochen2024compilation} also utilizes transfers but further improves scalability and fidelity by decomposing the compilation problem into standard optimization sub-problems and applying efficient heuristics to achieve near-optimal solutions.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{Figure/FidelityIntro.pdf}
    \vspace{-6pt}
    \caption{Error component of Enola and~\frameworkname.}
    \Description{Constraints}
    \label{fig:fidelityIntro} 
\end{figure}

While Enola has made significant progress, our error analysis reveals that there remains considerable room for further optimization. The error breakdown of Enola on the MaxCut QAOA benchmark is shown in Fig.\ref{fig:fidelityIntro}(a), consisting of four components: \emph{two-qubit gates}, \emph{Rydberg excitation}, \emph{qubit transfer}, and \emph{decoherence} (see Sec.\ref{sec:background} for more details on these error mechanisms). Among them, the two-qubit gate error has limited potential for further reduction since Enola does not introduce additional ones. However, the other three error components are not effectively mitigated and become dominant as the problem size increases, as Fig.\ref{fig:fidelityIntro}(a) shows. 

Nevertheless, these three error sources can actually be further controlled. Based on a thorough analysis on the limitation of the prior work (Sec.~\ref{subsec:limitation}), we identify a key reason for their sub-optimal performance: the \emph{limited exploitation of dynamic layout}---these approaches either use partially fixed layout essentially or restricts the flexibility of layout rearrangement. This limitation leads to more movements than actually needed, introducing excessive time overhead and transfers that finally contribute to the decoherence and transfer error. Moreover, we identify that the newly proposed ZA is promising for removing the excitation error, which arises from non-interacting qubits excited along with the interacting ones. This is achieved by moving non-interacting qubits back to storage during excitation. Due to its recent emergence, the prior work has not explored this possibility.

, but their limited utilization of dynamic layout also restricts them to incorporate this new feature, because ZA requires a higher level of inter-zone layout rearrangement.

This motivates us to propose a solution that fully uses the dynamic layout rearrangement, and ZA to avoid excitation error. However, achieving these goals is challenging. \textbf{First}, constantly changing the layout using movement not only needs to handle the conflict between the single qubit moves due to the constraints, but also need to prevent qubits from clustering and inducing unwanted interactions (more details in Sec.~\ref{sec:Motivate}). Handling these complexities simultaneously is hard. Therefore, the existing methods usually first fix a qubit layout and then focus on addressing the movement conflicts. ~\cite{tan2022qubit, tan2024compiling} try to address them at the same time by encoding these concerns into constraints and use solver-based method, but suffers from scalability issue. \textbf{Second,} 



% (Notably, single-qubit gate errors are excluded from this analysis, as they can be efficiently executed without introducing side effects and remain consistent across comparisons.)

% \noindent\textbf{Decoherence and transfer errors} primarily result from suboptimal movement scheduling. Enola predefines a qubit layout, where each collective movement modifies the layout for interaction and then returns the qubits to their original positions before the next movement. This back-and-forth scheme unnecessarily prolongs the movement time and increases transfers, worsening decoherence and transfer errors.

% \noindent\textbf{Rydberg excitation error} arises when non-interacting qubits are excited along with the interacting ones. Although Enola attempts to reduce the number of excitations, more qubits are inevitably excited as the problem size grows, amplifying this error.

To this end, we propose~\frameworkname, an innovative movement-based focusing on optimizing the overall fidelity on NAQC by effectively exploiting its qubit movement capabilities and ZA. Our solution (1) Continuous routing (multiple moves, then excite, this ), (2) Storage zone, (3) Multi-AOD to further boost the efficiency.


can potentially be circumvented by moving no-interaction qubits into storage zone using the newly demonstrated zoned architecture (ZA). However, the movement scheme of Enola cannot handle this design due to its partially fixed layout.

Our evaluation shows that


To best of our knowledge, our framework is the first to explore and optimize for the newly developed zoned architecture (ZA).


  
% In high level, this is due to the limit exploitation of the dynamic layout capability of NAQC.



We clarify collective movements, and Rydberg excitation

their methods fail to accommodate this inter-zone movement, because of the long-distance inter-zone movement... only maximize parallelism but overlook the distance...


% Each two-qubit gate has fidelity $99.5\%$, decoherence error scales with the program’s execution time which mainly consists of the movement time, each qubit transfer carries a $0.1\%$ risk of atom loss, and each Rydberg causes qubits not involved in interactions to experience a fidelity drop to around $99.75\%$ (see Sec.~\ref{sec:background} for more details on these error mechanisms).





To summarize, our contribution of this paper is as follows:
\begin{itemize}
    \item sss\\
    \item dd
\end{itemize}



%Unify the computing paradigm for near-term applications on bare qubits and long-term ones on logical qubits encoded in QEC codes.



% Promising as it may seem, effectively harnessing these advantages poses great challenge due to the constraints of qubit movement (more details in Sec.~\ref{sec:background}). \textbf{First}, the qubits can be collectively moved, but must be held in a 2D lattice frame, with the relative orders of rows and columns fixed throughout the movement due to the mechanism of their controlling optical tools~\cite{bluvstein2022quantum}. As a result, not all desired single qubit movements can be performed simultaneously within a frame, but have to be scheduled into different collective movements. \textbf{Second}, each collective movement involves picking up new qubits into the frame and drop old qubits to fixed positions, to obtain a desired layout rearrangement. This process of transferring qubits back and forth between \emph{static} to \emph{mobile} status induces time overhead along with risk of atom loss, thereby should be minimized. \textbf{Third}, the movement speed is restricted below some threshold to avoid atom heating that may let atom escape from the optical trap or corrupt the quantum state. Therefore, the distance of movements should be minimized to suppress the total movement time, which reduces the decoherence error and improves the output fidelity.

==> TexFile/02_Intro_02.tex <==
\section{Introduction}\label{sec:intro}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.99\textwidth]{Figure/IntroFig2.pdf}
    \caption{(a) Parallel CZ gate execution by placing interacting qubit pairs close together, enabled by the qubit movement feature (red circles). Non-interacting qubits in the computation zone experience excitation errors (blue circles). (b) Enola’s movement approach: reverting to the previous layout before rearranging to the next one, leading to higher transfer and decoherence errors. (c) Overview of the \frameworkname~framework. The \emph{Continuous Router} directly transitions between desired layouts without reverting to intermediate layouts. The \emph{Stage Scheduler} and \emph{Coll-Move Scheduler} coordinate inter-zone and intra-zone movements to maximize overall fidelity. All components support the integration of the storage zone.}
    \Description{Intro.}
    \label{fig:introfig}
    % \vspace{-2pt}
\end{figure*}

Quantum computing (QC) is swiftly evolving from a theoretical concept into a tangible reality, with significant advancements across various platforms over the past few decades~\cite{arute2019quantum, huang2020superconducting, bravyi2022future, bruzewicz2019trapped, chen2023benchmarking, kok2007linear, bourassa2021blueprint, bluvstein2024logical, wurtz2023aquila}. Given the rapid progress and the unique strengths of each platform, competition among these platforms is expected to persist for the foreseeable future.

Recently, \emph{neutral atom-based quantum computer (NAQC)}~\cite{ebadi2021quantum, graham2022multi, wurtz2023aquila, bluvstein2024logical} have emerged as a strong candidate in the QC landscape, due to its unique hardware advantages. These include impressive scalability (supporting up to 6100 qubits) ~\cite{manetsch2024tweezer, ebadi2022quantum, wurtz2023aquila, ebadi2021quantum}, long coherence times of several seconds~\cite{evered2023high, young2020half, barnes2022assembly}, and high-fidelity operations~\cite{bluvstein2024logical, levine2022dispersive, bluvstein2022quantum, levine2019parallel, fu2022high, evered2023high}, with single-qubit rotations and two-qubit CZ gates achieving fidelities of up to 99.99\% and 99.5\%, respectively.
%owing to their distinct hardware advantages. NAQC systems offer impressive scalability, supporting hundreds~\cite{ebadi2022quantum, wurtz2023aquila, ebadi2021quantum} to $6100$ qubits~\cite{manetsch2024tweezer}, long coherence times of several seconds~\cite{evered2023high, young2020half, barnes2022assembly}, and high-fidelity single-qubit rotations~\cite{bluvstein2024logical, levine2022dispersive, bluvstein2022quantum} as well as two-qubit CZ gates~\cite{levine2019parallel, fu2022high, evered2023high}, achieving fidelities up to $99.99\%$ and $99.5\%$, respectively. 

Beyond these fundamental features, NAQC offers the compelling ability to move qubits collectively using \emph{AOD}~\cite{bluvstein2022quantum}, enabling non-local connectivity and dynamic layouts that open new avenues for enhancing computational efficiency. For instance, this capability allows parallel execution of CZ gates: once interacting qubit pairs are brought close together, a global Rydberg laser~\cite{levine2019parallel, evered2023high} can perform CZ gates between these pairs (red circles in Fig.\ref{fig:introfig}(a)). This dynamic control has led to the development of the zoned architecture (ZA)~\cite{bluvstein2024logical}, which divides the system into distinct zones for specific tasks, such as storage and computation (e.g., CZ gates), with qubits shuttled between them (Fig.\ref{fig:introfig}(c)). Similar to classical architectures with separate memory and processing units, this design enhances overall system performance. For instance, non-interacting qubits can be moved to the storage zone to avoid excitation errors induced by the Rydberg laser (blue circle in Fig.~\ref{fig:introfig}(a)), preserved with negligible decoherence.
%This culminates in the demonstration of the \emph{zoned architecture (ZA)}~\cite{bluvstein2024logical} that divides the system into distinct zones for specific tasks such as storage and entangling, with qubits shuttled between them--akin to the classical architectures with separate memory and processing units--improving overall system performance.

% \todo{separate basic features with qubit movement and ZA, introduce parallel CZ gates using figures(resolved)}

While promising, fully leveraging these advantages presents great challenges. \textbf{First,} qubit movements must adhere to several constraints (see Sec.~\ref{subsec: NA hardware cap}), which often prevents desired single-qubit (1Q) movements from being executed collectively in one step, requiring multiple collective movements (Coll-Moves) instead. Failing to manage these constraints effectively results in excessive Coll-Moves, increasing total movement time and decoherence error. \textbf{Second}, qubits must be strategically placed to enable parallel interactions (Sec.~\ref{subsec: NA hardware cap}). If interacting qubits are spaced too far apart or additional qubits are clustered together, the desired parallel execution of CZ gates cannot be achieved.  \textbf{Third,} integrating the ZA adds further complexity with inter-zone movements, which can be more time-consuming than intra-zone moves and require careful scheduling. Importantly, these complexities cannot be addressed separately. An optimized Coll-Move may efficiently transport qubits but fail to support the intended CZ gates, while an optimized qubit layout may allow for many parallel CZ gates but require excessive Coll-Moves to achieve. Handling these complexities simultaneously is a challenging task.

% \todo{match advantages with challenges. (1) Qubit movement matched with movement constraints, (2) Parallel CZ matched with strategic qubit position, (3) ZA storage zone avoiding excitation error matched with complex inter-zone movement(resolved)} 

Several compilers have been developed~\cite{wang2024atomique, wang2023q, tan2022qubit, tan2024compiling, bochen2024compilation} to address these challenges. Among them, the most recent, Enola~\cite{bochen2024compilation}, has made significant progress in improving both fidelity and scalability compared to earlier solutions. However, our error analysis reveals that there is still considerable room for further optimization. The error breakdown of Enola on the MaxCut QAOA benchmark, shown in Fig.\ref{fig:fidelityIntro}(a), highlights four key error components: \emph{two-qubit (2Q) gates}, \emph{Rydberg excitation}, \emph{qubit transfer}, and \emph{decoherence} (see Sec.\ref{sec:background} for more details on these error mechanisms). While the 2Q gate error has limited potential for further reduction, as Enola does not introduce additional 2Q gates, the other three error sources are not effectively mitigated and become increasingly dominant as the problem size grows. We identify two key factors in Enola that contribute to these error sources:

% The work~\cite{wang2024atomique, wang2023q} fix the roles of static and mobile qubits and use multiple mobile arrays, SWAP gates, or ancilla qubits to facilitate qubit interactions. While this partially fixed layout simplifies the problem and leads to an efficient heuristic solution, the additional gates introduced for routing significantly reduce fidelity. In contrast, the works~\cite{tan2022qubit, tan2024compiling} directly address these complexities by encoding them into Boolean constraints, providing a solver-based solution. This method introduces no extra gates and achieves a degree of optimality, but suffers from severe scalability issues. More recent Enola~\cite{bochen} reformulates the compilation problem into standard optimization sub-problems and uses efficient heuristics to find near-optimal solutions, improving both scalability and fidelity.

\noindent\textbf{(1) Suboptimal Movement Scheme.} Enola reverts to a fixed layout before transitioning to the next, as shown in Fig.\ref{fig:introfig}(b). The reason is that Enola focuses on moving interacting qubits together, but this may cause multiple qubit clustering at a single location, leading to unwanted interactions. To address this, Enola reverts to a layout where qubits are spatially separated, before bringing them back together for interaction (Fig.\ref{fig:introfig}(b)). However, this approach results in excessive movement time and qubit transfers, contributing to both \emph{decoherence} and \emph{transfer errors}.

\noindent\textbf{(2) Difficulty in Storage Zone Integration.} Enola’s framework is limited to a computation zone, where non-interacting qubits experience \emph{excitation errors} (Fig.~\ref{fig:introfig}(a)). However, Enola cannot efficiently integrate a storage zone that helps to avoid these errors. Its design of reverting to a fixed layout requires all qubits to return to the storage zone before being moved back to the computation zone, leading to significant movement overhead due to frequent inter-zone communication.

To overcome these limitations and further improve fidelity, we propose \textbf{\frameworkname}, a novel compilation framework for NAQC. Our objectives are twofold: (1) to enable direct transitions between desired layouts for CZ execution without relying on intermediate layouts, and (2) to fully leverage the storage zone while introducing minimal additional overhead—both of which are beyond the capabilities of existing compilers. We achieve these goals through three key components (Fig.~\ref{fig:introfig}(c)) and significantly reduce the errors (Fig.~\ref{fig:fidelityIntro}(b)):

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{Figure/FidelityIntro.pdf}
    \vspace{-6pt}
    \caption{Error components of Enola and~\frameworkname.}
    \Description{Constraints}
    \label{fig:fidelityIntro} 
\end{figure}

(1) \emph{Stage Scheduler.} It analyzes the set of interacting qubits for each stage of parallel CZ gates and determines the execution order that minimizes qubit interchange between the computation and storage zones, thereby reducing inter-zone movement overhead (see Sec.~\ref{sec:stage scheduler}).

(2) \emph{Continuous Router.} It simultaneously handles the complexities of movement constraints, qubit positioning, and inter/intra-zone coordination to enable \emph{direct transitions} between layouts. It first determines both inter/intra-zone movements for each qubit, ensuring the desired inter-zone transport and CZ interactions without unwanted clustering. These movements are then unified and grouped into Coll-Moves while complying with movement constraints (see Sec.~\ref{sec:conti router}).

(3) \emph{Coll-Move Scheduler}. After the Coll-Moves are determined by the Continuous Router, this component schedules their execution to maximize qubit dwell time in the storage zone, minimizing decoherence error. It also incorporates the scheduling of multiple AOD arrays to further enhance movement parallelism and reduce latency (see Sec.~\ref{sec:Move scheduler}).

% The evaluation shows that we achieve improvement of several orders of magnitude in overall fidelity and 1.71x to 3.46x better compiled program execution time on average over a variety of benchmarks, using fewer compilation time by about 4x. 

Our evaluation shows improvements of several orders of magnitude in overall fidelity, with enhancements in compiled program execution time ranging from 1.71x to 3.46x across various benchmarks, alongside a reduction in compilation time by approximately 4x.

% However, transitioning directly between these optimized layouts is complex (see Sec.~\ref{subsec: our motivation}), so the solution reverts to an intermediate fixed layout before rearranging for the next one, resulting in large movement overhead and decoherence error. As Fig.~\ref{fig:fidelityIntro}(a) shows, decoherence becomes the dominant error source, especially in large-scale problems.

% These limitations highlight the difficulty of addressing the aforementioned complexities.

%However, minimize the groups of parallel CZ gates, maximizes the parallelism of CZ execution by transforming to layouts that



% Moreover, the movement scheme of Enola makes it hard to integrate the storage zone.

% A more efficient solution is to directly transition between layouts optimized for parallel CZ gates, but this requires addressing the complexities of movement constraints and qubit placement holistically.

To summarize, our contribution of this paper is as follows:
\begin{itemize}
\item We propose \textbf{\frameworkname}, a novel compiler for NAQC that fully leverages qubit movement capabilities while seamlessly integrating the newly developed ZA.

\item We integrate the storage zone for the first time, effectively eliminating excitation errors while minimizing the associated overhead.

\item We introduce a continuous router that enables direct transitions between qubit layouts with the storage zone, significantly reducing movement overhead.


\item We establish a stage scheduler and a Coll-Move scheduler that fully exploit the storage zone’s advantages, minimizing decoherence.

\item Our evaluation reveals a substantial improvement in fidelity and a significant reduction in both compiled program execution time and compilation time compared to the efficient baseline, demonstrating scalability. For large-scale programs, it achieves a fidelity enhancement by several orders of magnitude over Enola. Additionally, it enhances the execution time of compiled programs by a factor of 1.71x to 3.46x, alongside a reduction of compilation time by approximately 4x.
\end{itemize}

% These components fully leverage movement capabilities and the ZA, effectively reducing various error sources, as shown in Fig.\ref{sec:intro}. 


% To the best of our knowledge, \frameworkname~is the first to explore and optimize the newly developed ZA. Furthermore, our approach uses highly efficient heuristic algorithms, ensuring short compilation times and the ability to handle large-scale problems.






  
% In high level, this is due to the limit exploitation of the dynamic layout capability of NAQC.



% We clarify collective movements, and Rydberg excitation

% their methods fail to accommodate this inter-zone movement, because of the long-distance inter-zone movement... only maximize parallelism but overlook the distance...


% Each two-qubit gate has fidelity $99.5\%$, decoherence error scales with the program’s execution time which mainly consists of the movement time, each qubit transfer carries a $0.1\%$ risk of atom loss, and each Rydberg causes qubits not involved in interactions to experience a fidelity drop to around $99.75\%$ (see Sec.~\ref{sec:background} for more details on these error mechanisms).


%Unify the computing paradigm for near-term applications on bare qubits and long-term ones on logical qubits encoded in QEC codes.



% Promising as it may seem, effectively harnessing these advantages poses great challenge due to the constraints of qubit movement (more details in Sec.~\ref{sec:background}). \textbf{First}, the qubits can be collectively moved, but must be held in a 2D lattice frame, with the relative orders of rows and columns fixed throughout the movement due to the mechanism of their controlling optical tools~\cite{bluvstein2022quantum}. As a result, not all desired single qubit movements can be performed simultaneously within a frame, but have to be scheduled into different collective movements. \textbf{Second}, each collective movement involves picking up new qubits into the frame and drop old qubits to fixed positions, to obtain a desired layout rearrangement. This process of transferring qubits back and forth between \emph{static} to \emph{mobile} status induces time overhead along with risk of atom loss, thereby should be minimized. \textbf{Third}, the movement speed is restricted below some threshold to avoid atom heating that may let atom escape from the optical trap or corrupt the quantum state. Therefore, the distance of movements should be minimized to suppress the total movement time, which reduces the decoherence error and improves the output fidelity.

% Nevertheless, these three error sources can actually be further controlled. Based on a thorough analysis on the limitation of the prior work (Sec.~\ref{subsec:limitation}), we identify a key reason for their sub-optimal performance: the \emph{limited exploitation of dynamic layout}---these approaches either use partially fixed layout essentially or restricts the flexibility of layout rearrangement. This limitation leads to more movements than actually needed, introducing excessive time overhead and transfers that finally contribute to the decoherence and transfer error. 

% Moreover, we identify that the newly proposed ZA is promising for removing the excitation error, which arises from non-interacting qubits excited along with the interacting ones. This is achieved by moving non-interacting qubits back to storage during excitation. Due to its recent emergence, the prior work has not explored this possibility.

% , but their limited utilization of dynamic layout also restricts them to incorporate this new feature, because ZA requires a higher level of inter-zone layout rearrangement.

% This motivates us to propose a solution that fully uses the dynamic layout rearrangement, and ZA to avoid excitation error. However, achieving these goals is challenging. \textbf{First}, constantly changing the layout using movement not only needs to handle the conflict between the single qubit moves due to the constraints, but also need to prevent qubits from clustering and inducing unwanted interactions (more details in Sec.~\ref{sec:Motivate}). Handling these complexities simultaneously is hard. Therefore, the existing methods usually first fix a qubit layout and then focus on addressing the movement conflicts. ~\cite{tan2022qubit, tan2024compiling} try to address them at the same time by encoding these concerns into constraints and use solver-based method, but suffers from scalability issue. \textbf{Second,} 



% (Notably, single-qubit gate errors are excluded from this analysis, as they can be efficiently executed without introducing side effects and remain consistent across comparisons.)

% \noindent\textbf{Decoherence and transfer errors} primarily result from suboptimal movement scheduling. Enola predefines a qubit layout, where each collective movement modifies the layout for interaction and then returns the qubits to their original positions before the next movement. This back-and-forth scheme unnecessarily prolongs the movement time and increases transfers, worsening decoherence and transfer errors.

% \noindent\textbf{Rydberg excitation error} arises when non-interacting qubits are excited along with the interacting ones. Although Enola attempts to reduce the number of excitations, more qubits are inevitably excited as the problem size grows, amplifying this error.

==> TexFile/02_Intro_03.tex <==
\section{Introduction}\label{sec:intro}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.99\textwidth]{Figure/IntroFig1015.pdf}
    \caption{Overview of the \frameworkname~framework. The \emph{Continuous Router} enables directly layout transitions . The \emph{Stage Scheduler} and \emph{Coll-Move Scheduler} coordinate inter-zone and intra-zone movements to maximize overall fidelity. All components consider interplay of multiple constraints.}
    \Description{Intro.}
    \label{fig:introfig}
    % \vspace{-2pt}
\end{figure*}

Quantum computing (QC) is swiftly evolving from a theoretical concept into a tangible reality, with significant advancements across various platforms over the past few decades~\cite{arute2019quantum, huang2020superconducting, bravyi2022future, bruzewicz2019trapped, chen2023benchmarking, kok2007linear, bourassa2021blueprint, bluvstein2024logical, wurtz2023aquila}. Given the rapid progress and the unique strengths of each platform, competition among these platforms is expected to persist for the foreseeable future.

In recent years, \emph{neutral atom-based quantum computer (NAQC)}~\cite{ebadi2021quantum, graham2022multi, wurtz2023aquila, bluvstein2024logical} have emerged as a strong candidate in the QC landscape, due to its unique hardware advantages. These include impressive scalability (supporting up to 6100 qubits) ~\cite{manetsch2024tweezer, ebadi2022quantum, wurtz2023aquila, ebadi2021quantum}, long coherence times of several seconds~\cite{evered2023high, young2020half, barnes2022assembly}, and high-fidelity operations~\cite{bluvstein2024logical, levine2022dispersive, bluvstein2022quantum, levine2019parallel, fu2022high, evered2023high}, with single-qubit rotations and two-qubit CZ gates achieving fidelities of up to 99.99\% and 99.5\%, respectively.
%owing to their distinct hardware advantages. NAQC systems offer impressive scalability, supporting hundreds~\cite{ebadi2022quantum, wurtz2023aquila, ebadi2021quantum} to $6100$ qubits~\cite{manetsch2024tweezer}, long coherence times of several seconds~\cite{evered2023high, young2020half, barnes2022assembly}, and high-fidelity single-qubit rotations~\cite{bluvstein2024logical, levine2022dispersive, bluvstein2022quantum} as well as two-qubit CZ gates~\cite{levine2019parallel, fu2022high, evered2023high}, achieving fidelities up to $99.99\%$ and $99.5\%$, respectively. 

Beyond these fundamental features, NAQC offers the compelling ability to move qubits collectively using \emph{AOD} under some constraints~\cite{bluvstein2022quantum}, enabling non-local connectivity and dynamic layouts that facilitate parallel execution of CZ gates. Once interacting qubit pairs are brought close together, a global Rydberg laser\cite{levine2019parallel, evered2023high} can perform CZ gates between each pair (red circles in Fig.\ref{fig:introfig}(a)). This dynamic control has led to the development of the Zoned Architecture (ZA)~\cite{bluvstein2024logical}, which divides the system into distinct zones for specific tasks, such as storage and computation (e.g., CZ gates), with qubits shuttled between zones as needed (Fig.\ref{fig:introfig}(c)). Similar to classical architectures with separate memory and processing units, this design may enhance overall system performance. For example, non-interacting qubits can be moved to a storage zone, where they are preserved with negligible decoherence and are protected from excitation errors induced by the Rydberg laser (blue circle in Fig.\ref{fig:introfig}(a)).
% that open new avenues for enhancing computational efficiency. For instance, this capability allows
%This culminates in the demonstration of the \emph{zoned architecture (ZA)}~\cite{bluvstein2024logical} that divides the system into distinct zones for specific tasks such as storage and entangling, with qubits shuttled between them--akin to the classical architectures with separate memory and processing units--improving overall system performance.

% \todo{separate basic features with qubit movement and ZA, introduce parallel CZ gates using figures(resolved)}

% \todo{match advantages with challenges. (1) Qubit movement matched with movement constraints, (2) Parallel CZ matched with strategic qubit position, (3) ZA storage zone avoiding excitation error matched with complex inter-zone movement(resolved)} 

Several compilers have been developed~\cite{wang2024atomique, wang2023q, tan2022qubit, tan2024compiling, bochen2024compilation} to harness NAQC’s qubit movement capabilities. While these approaches have made remarkable progress, they still fall short of effectively exploiting the flexibility that qubit movement offers. \todo{Ideally, ... }They either settle for a partially fixed layout~\cite{wang2024atomique, wang2023q, bochen2024compilation} or struggle to handle fully dynamic layout transitions in a scalable manner~\cite{tan2022qubit, tan2024compiling}. As a result, there remains significant room for further improvement. \todo{maybe revise this part a little bit to include Enola? This would help pave the way for focusing the comparasion with Enola?}
\todo{previous work has no ZA, they cannot be easily extended to ZA}
\todo{Formulate the problem/revisit the design space, briefly introduce four key components, large design space but can still handle}
We identified a fundamental reason behind these limitations: previous methods address the constraints of the problem separately, missing key optimization opportunities that stem from their interdependencies. For example, approaches like~\cite{wang2024atomique, wang2023q, bochen2024compilation} first handle qubit allocation to determine an initial layout, and then optimize qubit movements based on that layout. This locks the movement scheme into a fixed initial layout, restricting flexibility in layout transitions. Simultaneously addressing qubit allocation and movement would unlock the full potential of dynamic layout transitions. On the other hand, solver-based methods~\cite{tan2022qubit, tan2024compiling} simply encode all constraints without leveraging their interdependencies, leading to scalability challenges.

%highlighting the difficulty of effectively managing these complexities simultaneously.


% we first identified two key complexities in the NAQC compilation problem. (1) \emph{Qubit allocation.} Qubits must be placed strategically to enable desired CZ gates while avoiding unwanted interactions. (2) \emph{Movement constraints.} Qubit movements must follow specific rules~\cite{bluvstein2024logical, bluvstein2022quantum} to be grouped into collective movements. The essential reason for the limitation of existing work is that they address these complexities in isolation, missing crucial optimization opportunities that arise from their interdependencies. For example, heuristic methods like~\cite{wang2024atomique, wang2023q, bochen2024compilation} optimize the qubit allocation and movements separately, leading to a movement scheme based on a partially fixed layout.

% Movement can change the qubit positions, and the qubits with locations already decided can guide the movement of the remaining qubits.

Building on these insights, we developed \textbf{\frameworkname}, a NAQC compiler that holistically addresses various constraints, fully leveraging their interplay to unlock new optimization opportunities. We identified \emph{four} key categories of constraints in the NAQC compilation problem: (1) \emph{Gate scheduling}, (2) \emph{Qubit allocation}, (3) \emph{Qubit movement}, and (4) \emph{Storage zone}. Based on these, we designed \emph{three} core components that make up our solution. Each component considers multiple constraint categories, exploiting their interdependencies to achieve more effective optimization, as Fig.~\ref{fig:introfig} illustrates. These components are:
\todo{Answer a question: why can we still manage a larger design space?}
\noindent (1) \emph{Stage Scheduler.} It partitions CZ gates into stages of parallel execution and schedule the order of execution to minimize qubit interchange between the computation and storage zones, reducing inter-zone movement overhead (see Sec.~\ref{sec:stage scheduler}).

\noindent (2) \emph{Continuous Router.} It enables \emph{continuous transitions} between layouts, eliminating the need for intermediate fixed layouts. This is achieved through an efficient heuristic that simultaneously manages qubit allocation, movement constraints, and inter-zone coordination (see Sec.~\ref{sec:conti router}).

\noindent (3) \emph{Coll-Move Scheduler.} It optimizes the execution order of collective movements to maximize qubit dwell time in the storage zone, minimizing decoherence. It also incorporates the scheduling of multiple AOD arrays to further enhance movement parallelism and reduce latency (see Sec.~\ref{sec:Move scheduler}).


% either settle for a partially fixed layout~\cite{wang2024atomique, wang2023q, bochen2024compilation} or struggle to handle fully dynamic layout transitions in a scalable way~\cite{tan2022qubit, tan2024compiling}, 

% For example, heuristic methods like~\cite{wang2024atomique, wang2023q, bochen2024compilation} optimize qubit allocation and movement constraints separately, leading to a partially fixed layout that restricts dynamic flexibility. Conversely, solver-based methods like~\cite{tan2022qubit, tan2024compiling} encode all complexities into constraints but face scalability issues, highlighting the difficulty of effectively managing these complexities simultaneously.


% (3) \emph{Inter-zone coordination.} Minimizing costly inter-zone movements and scheduling them efficiently with intra-zone ones is essential to reduce latency. 

%Existing approaches often address these challenges in isolation, missing crucial optimization opportunities that arise from their interdependencies.

%our error analysis reveals that 

% The work~\cite{wang2024atomique, wang2023q} fix the roles of static and mobile qubits and use multiple mobile arrays, SWAP gates, or ancilla qubits to facilitate qubit interactions. While this partially fixed layout simplifies the problem and leads to an efficient heuristic solution, the additional gates introduced for routing significantly reduce fidelity. In contrast, the works~\cite{tan2022qubit, tan2024compiling} directly address these complexities by encoding them into Boolean constraints, providing a solver-based solution. This method introduces no extra gates and achieves a degree of optimality, but suffers from severe scalability issues. More recent Enola~\cite{bochen} reformulates the compilation problem into standard optimization sub-problems and uses efficient heuristics to find near-optimal solutions, improving both scalability and fidelity.

% While promising, fully leveraging these advantages presents great challenges. \textbf{First,} qubit movements must adhere to several constraints (see Sec.~\ref{subsec: NA hardware cap}), which often prevents desired single-qubit (1Q) movements from being executed collectively in one step, requiring multiple collective movements (Coll-Moves) instead. Failing to manage these constraints effectively results in excessive Coll-Moves, increasing total movement time and decoherence error. \textbf{Second}, qubits must be strategically placed to enable parallel interactions (Sec.~\ref{subsec: NA hardware cap}). If interacting qubits are spaced too far apart or additional qubits are clustered together, the desired parallel execution of CZ gates cannot be achieved.  \textbf{Third,} integrating the ZA adds further complexity with inter-zone movements, which can be more time-consuming than intra-zone moves and require careful scheduling. Importantly, these complexities cannot be addressed separately. An optimized Coll-Move may efficiently transport qubits but fail to support the intended CZ gates, while an optimized qubit layout may allow for many parallel CZ gates but require excessive Coll-Moves to achieve. Handling these complexities simultaneously is a challenging task.

% \noindent\textbf{(1) Suboptimal Movement Scheme.} Enola reverts to a fixed layout before transitioning to the next, as shown in Fig.\ref{fig:introfig}(b). The reason is that Enola focuses on moving interacting qubits together, but this may cause multiple qubit clustering at a single location, leading to unwanted interactions. To address this, Enola reverts to a layout where qubits are spatially separated, before bringing them back together for interaction (Fig.\ref{fig:introfig}(b)). However, this approach results in excessive movement time and qubit transfers, contributing to both \emph{decoherence} and \emph{transfer errors}.

% \noindent\textbf{(2) Difficulty in Storage Zone Integration.} Enola’s framework is limited to a computation zone, where non-interacting qubits experience \emph{excitation errors} (Fig.~\ref{fig:introfig}(a)). However, Enola cannot efficiently integrate a storage zone that helps to avoid these errors. Its design of reverting to a fixed layout requires all qubits to return to the storage zone before being moved back to the computation zone, leading to significant movement overhead due to frequent inter-zone communication.

% Building on these insights, we propose \textbf{\frameworkname}, a novel compilation framework for NAQC that holistically addresses the complexities of the problem, leveraging their interdependencies to unlock new optimization opportunities. This approach is realized through three key components (Fig.~\ref{fig:introfig}(c)):


%We manage to enable direct transitions between desired layouts for CZ execution, fully utilizing the dynamic layout capability. Moreover, this framework seamlessly integrates a storage zone by coordinating inter- and intra-moves in a unifying approach, which is beyond the scope of existing compilers. 

%Notably, we for the first time exploit the ZA in NAQC compiler. Notably, the design of these components take multiple complexities into consideration 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{Figure/FidelityIntro.pdf}
    \vspace{-6pt}
    \caption{Error components of Enola and~\frameworkname.}
    \Description{Constraints}
    \label{fig:fidelityIntro} 
\end{figure}

% It first determines both inter/intra-zone movements for each qubit, ensuring the desired inter-zone transport and CZ interactions without unwanted clustering. These movements are then unified and grouped into Coll-Moves while complying with movement constraints (see Sec.~\ref{sec:conti router}).

% (1) \emph{Stage Scheduler.} It analyzes the set of interacting qubits for each stage of parallel CZ gates and determines the execution order that minimizes qubit interchange between the computation and storage zones, thereby reducing inter-zone movement overhead (see Sec.~\ref{sec:stage scheduler}).

% (2) \emph{Continuous Router.} It simultaneously handles the complexities of movement constraints, qubit positioning, and inter/intra-zone coordination to enable \emph{direct transitions} between layouts. It first determines both inter/intra-zone movements for each qubit, ensuring the desired inter-zone transport and CZ interactions without unwanted clustering. These movements are then unified and grouped into Coll-Moves while complying with movement constraints (see Sec.~\ref{sec:conti router}).

% (3) \emph{Coll-Move Scheduler}. After the Coll-Moves are determined by the Continuous Router, this component schedules their execution to maximize qubit dwell time in the storage zone, minimizing decoherence error. It also incorporates the scheduling of multiple AOD arrays to further enhance movement parallelism and reduce latency (see Sec.~\ref{sec:Move scheduler}).

%, and (2) to fully leverage the storage zone while introducing minimal additional overhead—both of which are beyond the capabilities of existing compilers. 

% The error breakdown of Enola on the MaxCut QAOA benchmark, shown in Fig.\ref{fig:fidelityIntro}(a), highlights four key error components: \emph{two-qubit (2Q) gates}, \emph{Rydberg excitation}, \emph{qubit transfer}, and \emph{decoherence} (see Sec.\ref{sec:background} for more details on these error mechanisms). While the 2Q gate error has limited potential for further reduction, as Enola does not introduce additional 2Q gates, the other three error sources are not effectively mitigated and become increasingly dominant as the problem size grows. We identify two key factors in Enola that contribute to these error sources:

% The evaluation shows that we achieve improvement of several orders of magnitude in overall fidelity and 1.71x to 3.46x better compiled program execution time on average over a variety of benchmarks, using fewer compilation time by about 4x. 

Our evaluation demonstrates improvements of several orders of magnitude in overall fidelity compared to the state-of-the-art approach, Enola~\cite{bochen2024compilation}, as shown in Fig.~\ref{fig:fidelityIntro}(b). Additionally, \frameworkname~achieves execution time enhancements ranging from 1.71x to 3.46x across various benchmarks, along with a reduction in compilation time by up to 213.5x.

% However, transitioning directly between these optimized layouts is complex (see Sec.~\ref{subsec: our motivation}), so the solution reverts to an intermediate fixed layout before rearranging for the next one, resulting in large movement overhead and decoherence error. As Fig.~\ref{fig:fidelityIntro}(a) shows, decoherence becomes the dominant error source, especially in large-scale problems.

% These limitations highlight the difficulty of addressing the aforementioned complexities.

%However, minimize the groups of parallel CZ gates, maximizes the parallelism of CZ execution by transforming to layouts that



% Moreover, the movement scheme of Enola makes it hard to integrate the storage zone.

% A more efficient solution is to directly transition between layouts optimized for parallel CZ gates, but this requires addressing the complexities of movement constraints and qubit placement holistically.

To summarize, our contribution of this paper is as follows:
\begin{itemize}
\item We propose \textbf{\frameworkname}, a novel compiler for NAQC that fully leverages qubit movement capabilities while seamlessly integrating the newly developed ZA.

\item We integrate the storage zone for the first time, effectively eliminating excitation errors while minimizing the associated overhead.

\item We introduce a continuous router that enables direct transitions between qubit layouts with the storage zone, significantly reducing movement overhead.


\item We establish a stage scheduler and a Coll-Move scheduler that fully exploit the storage zone’s advantages, minimizing decoherence.

\item Our evaluation reveals substantial improvements in fidelity, along with significant reductions in both execution time and compilation time compared to the state-of-the-art baseline.
% For large-scale programs, it achieves a fidelity enhancement by several orders of magnitude over Enola. Additionally, it enhances the execution time of compiled programs by a factor of 1.71x to 3.46x, alongside a reduction of compilation time by approximately up to 213.5x.
\end{itemize}

% These components fully leverage movement capabilities and the ZA, effectively reducing various error sources, as shown in Fig.\ref{sec:intro}. 


% To the best of our knowledge, \frameworkname~is the first to explore and optimize the newly developed ZA. Furthermore, our approach uses highly efficient heuristic algorithms, ensuring short compilation times and the ability to handle large-scale problems.






  
% In high level, this is due to the limit exploitation of the dynamic layout capability of NAQC.



% We clarify collective movements, and Rydberg excitation

% their methods fail to accommodate this inter-zone movement, because of the long-distance inter-zone movement... only maximize parallelism but overlook the distance...


% Each two-qubit gate has fidelity $99.5\%$, decoherence error scales with the program’s execution time which mainly consists of the movement time, each qubit transfer carries a $0.1\%$ risk of atom loss, and each Rydberg causes qubits not involved in interactions to experience a fidelity drop to around $99.75\%$ (see Sec.~\ref{sec:background} for more details on these error mechanisms).


%Unify the computing paradigm for near-term applications on bare qubits and long-term ones on logical qubits encoded in QEC codes.



% Promising as it may seem, effectively harnessing these advantages poses great challenge due to the constraints of qubit movement (more details in Sec.~\ref{sec:background}). \textbf{First}, the qubits can be collectively moved, but must be held in a 2D lattice frame, with the relative orders of rows and columns fixed throughout the movement due to the mechanism of their controlling optical tools~\cite{bluvstein2022quantum}. As a result, not all desired single qubit movements can be performed simultaneously within a frame, but have to be scheduled into different collective movements. \textbf{Second}, each collective movement involves picking up new qubits into the frame and drop old qubits to fixed positions, to obtain a desired layout rearrangement. This process of transferring qubits back and forth between \emph{static} to \emph{mobile} status induces time overhead along with risk of atom loss, thereby should be minimized. \textbf{Third}, the movement speed is restricted below some threshold to avoid atom heating that may let atom escape from the optical trap or corrupt the quantum state. Therefore, the distance of movements should be minimized to suppress the total movement time, which reduces the decoherence error and improves the output fidelity.

% Nevertheless, these three error sources can actually be further controlled. Based on a thorough analysis on the limitation of the prior work (Sec.~\ref{subsec:limitation}), we identify a key reason for their sub-optimal performance: the \emph{limited exploitation of dynamic layout}---these approaches either use partially fixed layout essentially or restricts the flexibility of layout rearrangement. This limitation leads to more movements than actually needed, introducing excessive time overhead and transfers that finally contribute to the decoherence and transfer error. 

% Moreover, we identify that the newly proposed ZA is promising for removing the excitation error, which arises from non-interacting qubits excited along with the interacting ones. This is achieved by moving non-interacting qubits back to storage during excitation. Due to its recent emergence, the prior work has not explored this possibility.

% , but their limited utilization of dynamic layout also restricts them to incorporate this new feature, because ZA requires a higher level of inter-zone layout rearrangement.

% This motivates us to propose a solution that fully uses the dynamic layout rearrangement, and ZA to avoid excitation error. However, achieving these goals is challenging. \textbf{First}, constantly changing the layout using movement not only needs to handle the conflict between the single qubit moves due to the constraints, but also need to prevent qubits from clustering and inducing unwanted interactions (more details in Sec.~\ref{sec:Motivate}). Handling these complexities simultaneously is hard. Therefore, the existing methods usually first fix a qubit layout and then focus on addressing the movement conflicts. ~\cite{tan2022qubit, tan2024compiling} try to address them at the same time by encoding these concerns into constraints and use solver-based method, but suffers from scalability issue. \textbf{Second,} 



% (Notably, single-qubit gate errors are excluded from this analysis, as they can be efficiently executed without introducing side effects and remain consistent across comparisons.)

% \noindent\textbf{Decoherence and transfer errors} primarily result from suboptimal movement scheduling. Enola predefines a qubit layout, where each collective movement modifies the layout for interaction and then returns the qubits to their original positions before the next movement. This back-and-forth scheme unnecessarily prolongs the movement time and increases transfers, worsening decoherence and transfer errors.

% \noindent\textbf{Rydberg excitation error} arises when non-interacting qubits are excited along with the interacting ones. Although Enola attempts to reduce the number of excitations, more qubits are inevitably excited as the problem size grows, amplifying this error.

==> TexFile/03_Background_01.tex <==
\section{Background}\label{sec:background}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.99\textwidth]{Figure/Background1.pdf}
    \caption{Illustration of capabilities of NA hardware based on zoned architecture.}
    \Description{Background. NA hardware capabilities.}
    \label{fig:background}
    % \vspace{-2pt}
\end{figure*}

This section provides essential background information on NA hardware capabilities, along with a brief introduction on the existing NA compilers.

\subsection{NA Hardware Capabilities}
\todo{Need to revise, shorter}
We first introduce the gate operations of NA hardware.

\noindent\textbf{Gate Operations. }NAQC supports high-fidelity single-qubit rotations (1Q gates) and CZ gates, which are sufficient for universal quantum computing~\cite{boykin1999universal}. \emph{1Q gates} are implemented using qubit-specific, parallel Raman pulses with fidelities $99.99\%$ and duration $\sim 1 \mu s$~\cite{bluvstein2022quantum, levine2022dispersive, evered2023high, bluvstein2024logical}. This allows for reliable simultaneous 1Q gate execution across the entire qubit plane, as illustrated by the vertical red beams in Fig.~\ref{fig:background}.


The \emph{CZ gate} are performed by positioning qubits within Rydberg radius ($r_b \approx 6 \mu m$~\cite{bochen2024compilation}) and applying a global Rydberg laser excitation (horizontal blue light in Fig.\ref{fig:background})~\cite{bluvstein2022quantum, bluvstein2024logical}. Atom pairs within $r_b$ undergo CZ gates through the Rydberg blockade effect~\cite{jaksch2000fast, urban2009observation, levine2019parallel}, while the other qubits need to be spaced far enough (>$10\mu m$~\cite{bluvstein2024logical}) to avoid unwanted interactions. Recent advancements have achieved competitive fidelities of $99.5\%$ with duration $270ns$~\cite{bluvstein2024logical}. This enables parallel execution of multiple CZ gates on distinct qubits, provided that they are wisely positioned.

\noindent\textbf{Excitation Error.} The non-interacting qubits will not experience a CZ gate during the Rydberg excitation, but will be excited to Rydberg state and return to the original state. This process introduces a fidelity drop to $99.75\%$~\cite{bochen2024compilation}.

% \noindent\textbf{(Mid-circuit) Measurement.} Measurement is performed using \emph{fluorescence imaging}, where an imaging laser causes atoms in specific states to fluoresce, while others remain dark, allowing qubit states to be determined based on fluorescence~\cite{shea2020submillisecond} (horizontal red light in Fig.~\ref{fig:background}). Mid-circuit measurement is achieved by moving selected qubits to a separate readout zone for measurement~\cite{bluvstein2022quantum}, among other methods~\cite{graham2023midcircuit, deist2022mid, singh2023mid, ma2023high, lis2023midcircuit}. The current readout time is $\sim 500 \mu s$ with a fidelity of $99.8\%$~\cite{bluvstein2024logical}, with potential improvements reducing the time to around $100 \mu s$~\cite{shea2020submillisecond}.

\begin{table}[htbp]
\centering
	\begin{tabular}{| c | c | c | c | c |}
	\hline
	    & 1Q Gate  & CZ Gate & Excitation & Transfer\\
	\hline
         Fidelity & $99.99\%$ & $99.5\%$ & $99.75\%$ & $99.9\%$\\
         \hline
         Duration & $1\mu s$ & $270ns$ & $270ns$ & $100\mu s$\\
         \hline
	\end{tabular}
 \centering
 \vspace{3pt}
\caption{Parameters on the fidelity and duration of operations on NAQC.}
\label{NA hardware parameter}
\end{table}

Second, we introduce NAQC's qubit movement feature through optical traps~\cite{beugnon2007two}.

\noindent\textbf{Optical Traps.} There are two types of optical traps: (1) \emph{static traps} generated by a spatial light modulator (SLM)~\cite{ebadi2021quantum, scholl2021quantum}, and (2) \emph{mobile traps} generated by a crossed 2D acousto-optic deflector (AOD)~\cite{bluvstein2022quantum}, represented by blue and yellow (or green) dots in Fig.\ref{fig:background}, respectively. These traps are typically arranged in a 2D lattice array. Qubits in SLM traps remain fixed, while those in AOD traps can be moved collectively subject to certain constraints (details in \emph{Movement Constraints} subsection). We refer to them as \emph{static qubits} and \emph{mobile qubits}.

\noindent\textbf{Trap Transfer.}
Qubits can be transferred between SLM and AOD traps with $0.1\%$ risk of atom loss and a duration of $100 \mu s$~\cite{bluvstein2024logical} (green dots in Fig.~\ref{fig:background}). The combined use of trap transfer and qubit movement allows for dynamic reconfiguration of the layout during computation.

\noindent\textbf{Movement Constraints.}
The collective movement in an AOD lattice must respect the following constraints (Fig.~\ref{fig:constraints}).\\ 
\noindent (1) \emph{Rows and columns must move in tandem.} This means that moving a qubit in an AOD array requires moving all qubits in the same row or column~\cite{bluvstein2022quantum}.\\
\noindent (2) \emph{Rows and columns cannot cross.} The AOD frame can stretch or contract in two directions, but the relative order of rows and columns must remain unchanged~\cite{bluvstein2022quantum}.\\
\noindent (3) \emph{Movement speed must be controlled.} According to experiments in~\cite{bluvstein2022quantum}, qubit fidelity is maintained as long as the speed does not exceed $0.55\mu m\cdot \mu s^{-1}$.

\noindent Notably, NAQC can support multiple independently operating AOD arrays, such as the yellow and green lattices. The qubit movements in distinct AOD arrays do not need to satisfy the above constraints.

\noindent\textbf{Qubit Interaction.} Interactions between qubits within an SLM array or an AOD array, between an SLM qubit and an AOD qubit, or between qubits from distinct AOD arrays are allowed when they are within the Rydberg radius $r_b$, as Fig.~\ref{fig:constraints} shows. Since SLM qubits are typically spaced at a safe distance ($>10\mu m$~\cite{bluvstein2024logical}) to avoid unintended interactions, SLM-SLM interactions require mediation via trap transfer~\cite{tan2024compiling, bochen2024compilation, tan2022qubit}, SWAP gates~\cite{wang2024atomique}, or ancillas qubits~\cite{wang2023q} for routing (more details in Sec.~\ref{subsec: NA comp}).

Finally, we introduce the \emph{zoned architecture (NA)}, which has been physically demonstrated recently~\cite{bluvstein2024logical}.

\noindent\textbf{Zoned Architecture.} The current ZA~\cite{bluvstein2024logical} divides the computational space into distinct zones for specific tasks. For instance, they set a storage zone where qubit state can be preserved with negligible decoherence, and an entangling zone dedicated for parallel CZ execution. Qubits can be shuttled between these zones as needed. Although originally designed for logical qubits in QEC codes~\cite{knill1997theory}, ZA also presents new opportunities for optimizing near-term applications with bare qubits.
%(The mid-circuit image is collected with a CMOS camera and sent to a field-programmable gate array (FPGA) for real-time decoding and feedforward.)
For more details of hardware features, please refer to~\cite{bluvstein2024logical, schmid2024computational, wurtz2023aquila}. We summarize the hardware parameters into Table~\ref{NA hardware parameter}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{Figure/AOD Constraints.pdf}
    \vspace{-6pt}
    \caption{Constraints on qubit movement and interaction.}
    \Description{Constraints}
    \label{fig:constraints} 
\end{figure}

\subsection{NA Compilers}\label{subsec: NA comp}
Current compiler typically decompose the compilation problem into several sub-problems: Qubit mapping and gate scheduling. They try to maximize parallel CZ gates by routing, using the qubit movement ability. However, in high level, the previous methods are limited in utilizing the dynamic layout of NAQC.

The work~\cite{wang2024atomique, wang2023q} keep a portion of qubits fixed throughout the computation and use SWAP gates combined with qubit movement for routing of distant static qubits, as shown in Fig.~\ref{}. Although..., this method introduce numerous two-qubit gates for routing, largely compromising the output fidelity. The work~\cite{tan2020optimal, tan2024compiling} solver-based, but enforce a Rydberg excitation after each collective movements (why?), introducing excessive excitation error. The improved work~\cite{bochen2024compilation} allows multiple collective movements between Rydberg excitations, but they reverse all the collective movements before the next stage, wasting lots of time. \todo{Do I need to say this here or in motivation?}

\iffalse
The main takeaways are:
(1) 1Q gates can be executed in parallel in any zone with very high fidelity and within a short duration. In contrast, the execution parallel CZ gates require moving the associated atoms into adjacent locations, and has much lower fidelity albeit with a comparable gate speed. Therefore, CZ gates are the primary error source for gate operations and their number should be minimized.

(2) Continuous provision of atom. Scalability is not an issue for near term applications. Ancilla qubits are affordable.

(3) Atom movement and measurement has high fidelity but are time-consuming. Therefore, they are not the main error source but their frequencies should be minimized to reduce the time overhead.

Movement with high parallelism in two dimensions

The qubits without interaction will still be excited by Rydberg laser and experience error. Therefore, we need to maximize the ratio of qubits under CZ interaction.

1Q Layer + CZ Block
\fi




% NAQC encodes qubits in the internal states of individual atoms, such as hyperfine states in alkali atoms~\cite{bluvstein2024logical,wurtz2023aquila} and nuclear spin in alkaline-earth-like atoms~\cite{ma2022universal, jenkins2022ytterbium}. These long-lived quantum states result in ultra-stable qubits with coherence times ranging from a few seconds to minutes~\cite{evered2023high, young2020half, barnes2022assembly}, making them ideal for robust quantum information storage. NAQCs can trap hundreds to thousands of atoms in optical lattices~\cite{ebadi2022quantum, wurtz2023aquila, manetsch2024tweezer} and selectively move them using \emph{optical tweezers}~\cite{beugnon2007two}, enabling reconfigurable qubit arrangements essential for scalable QC architectures. 

==> TexFile/04_Motivate_01.tex <==
\section{Motivation}\label{sec:Motivate}
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.99\textwidth]{Figure/Motivation.pdf}
    \caption{(a)-(d) Limitations of existing NA compilers compared to~\frameworkname. Our framework optimize the layout sequence and the number of excitations without introducing additional CZ gates, thereby improving overall fidelity. (e1)-(e4) Continuous routing challenges. (e2) Qubits may cluster at a single site, causing unwanted interactions. (e3) A simple solution is to return all qubits to their original positions before the next layout preparation, but this results in significant overhead. (e4) Our framework routes interacting qubits directly from the current layout to the next step, significantly reducing movement overhead.}
    \Description{NA compiler review.}
    \label{fig:motivation}
    % \vspace{-2pt}
\end{figure*}

This section first analyzes the limitations of current work (Sec.\ref{subsec:limitation}). Building on this, we introduce the key motivations behind our solution, which addresses these shortcomings (Sec.\ref{subsec: our motivation}). We provide examples to illustrate the challenges in achieving these goals, highlighting that they require non-trivial effort beyond the capabilities of existing approaches.

\subsection{Limitations of Existing NA Compilers}\label{subsec:limitation}
An overview of the current NA compilers is shown in Fig.~\ref{fig:motivation}, and we detail their limitations below.

\noindent\textbf{Fig.\ref{fig:motivation}(a)} shows the routing strategy of~\cite{wang2024atomique, wang2023q}. To enable interaction between distant static qubits ($q_1$, $q_2$), they first swap the state of static qubit $q_1$ to mobile qubit $q_3$, move $q_3$ to $q_2$, and then perform the CZ gate. Although they employ a well-established compiler~\cite{li2019tackling} to minimize SWAP gates and utilize multiple AOD arrays for inter-array interaction, the excessive gate insertion leads to significant fidelity loss.

\noindent\textbf{Fig.\ref{fig:motivation}(b)} shows the layout rearrangement strategy of~\cite{tan2022qubit, tan2024compiling}. They limit the process to one collective movement before each excitation, restricting the number of parallel CZ gates their layout can support. More collective movements could create additional close qubit pairs for interaction before each excitation. The suboptimal layouts, marked in grey, increase the number of excitations, leading to higher excitation error.

\noindent\textbf{Fig.\ref{fig:motivation}(c)} illustrates the strategy of~\cite{bochen2024compilation}, which allows multiple collective movements before each excitation, maximizing parallel CZ gates per excitation. These optimized layouts, marked in red, reduce the number of required excitations and the excitation error. However, they reverse the collective movements to return to the original layout before preparing for the next excitation, increasing both movement time and the number of transfers.

This analysis motivates the development of a solution that avoids additional CZ gates, minimizes the number of excitations, and optimizes layout rearrangement sequences. To achieve this, we utilize qubit transfers to eliminate extra CZ gates and employ multiple collective movements to directly transition between highly parallel CZ gate layouts (marked in red) without reverting to previous layouts (Fig.\ref{fig:motivation}(d)). Furthermore, the potential of the ZA has not been explored in prior work due to its recent emergence. Our solution aims to fully leverage the capabilities of ZA for enhanced performance. Sec.~\ref{subsec: our motivation} delves deeper into these concepts and highlights the challenges involved.
%so that the CZ gate error, excitation error, transfer error, and decoherence error are all effectively suppressed.

\subsection{Motivation of~\frameworkname}{\label{subsec: our motivation}}
%First of all, we adopt transfer to dynamically change qubit layout without introducing more CZ gates, because the $0.1\%$ risk of atom loss due to transfer is cheaper than introducing extra CZ gate with infidelity $0.5\%$. 

Based on our analysis of the limitations in prior work, we identify three key motivations for our framework, along with the challenges that make these goals difficult to achieve with existing solutions.

\noindent\textbf{1. Continuous Routing Improves Movement.} Our goal is to develop a movement framework that directly transitions between layouts, which we call \emph{continuous routing}. However, this is challenging due to the risk of clustering multiple qubits at one site, leading to unwanted interactions. For instance, Fig.\ref{fig:motivation} (e1) shows qubits $q_2$, $q_4$, and $q_6$ moving to interact with $q_1$, $q_3$, and $q_5$. In the next step, CZ gates are required between $(q_2, q_3)$ and $(q_4, q_5)$. Moving $q_2$ and $q_4$ to $q_3$ and $q_5$ seems logical, but clustering $q_4$, $q_5$, and $q_6$ at one site prevents the intended CZ gate between $(q_4, q_5)$ (Fig.~\ref{fig:motivation}(e2)). Solver-based compilers~\cite{tan2022qubit, tan2024compiling} address this by encoding constraints but face severe scalability issues. Other approaches, such as~\cite{bochen2024compilation}, group non-conflicting single-qubit movements but cannot address clustering issues. To avoid this risk, they revert to the original layout between rearrangements (Fig.~\ref{fig:motivation}(e3)), increasing both movement time and transfers. A viable solution, as shown in Fig.~\ref{fig:motivation}(e4), would involve moving interacting qubits to an empty site (e.g., $q_4, q_5$), but this added flexibility significantly expands the design space, making it more challenging to find an optimal solution.

\noindent\textbf{2. Storage Zone Avoids Excitation Error.}
To leverage the ZA, we propose moving non-interacting qubits from the entangling zone to the storage zone to avoid excitation errors, and only moving them back when CZ gates are required. This strategy, while promising, introduces more complexity due to inter-zone communication. Minimizing costly inter-zone movements and coordinating intra- and inter-zone activities are essential to reducing movement overhead— a challenge existing solutions cannot address. Directly applying the method from~\cite{bochen2024compilation} would fix all qubits in the storage zone, move interacting qubits to the entangling zone, and return them to storage after each excitation, leading to excessive inter-zone movements and decoherence errors.

\noindent\textbf{3. Multi-AODs Boost Parallelism.} While the work~\cite{wang2024atomique} used multiple AODs to increase parallelism via inter-array interactions, we find it more effective to use multiple AODs to execute several collective movements in parallel. Although single-qubit movements in different collective movements may conflict due to constraints, they can be executed simultaneously in different AODs, which operate independently. Achieving this requires a careful assignment of movements to AODs to minimize system latency. Prior work, limited to a single AOD, does not take advantage of this capability.

In summary, while the motivations for further improvements are clear, achieving these goals requires significant effort. Our solution addresses these challenges. We first provide an overview of our framework in Sec.~\ref{sec:overview}, followed by technical details in Sec.~\ref{sec:conti router},~\ref{sec:stage scheduler},~\ref{sec:multi-AOD scheduler}.

==> TexFile/04_Motivation_02.tex <==
\section{Motivation}\label{sec:Motivate}
% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=0.99\textwidth]{Figure/Motivation.pdf}
%     \caption{(a)-(d) Limitations of existing NA compilers compared to~\frameworkname. Our framework optimize the layout sequence and the number of excitations without introducing additional CZ gates, thereby improving overall fidelity. (e1)-(e4) Continuous routing challenges. (e2) Qubits may cluster at a single site, causing unwanted interactions. (e3) A simple solution is to return all qubits to their original positions before the next layout preparation, but this results in significant overhead. (e4) Our framework routes interacting qubits directly from the current layout to the next step, significantly reducing movement overhead.}
%     \Description{NA compiler review.}
%     \label{fig:motivation}
%     % \vspace{-2pt}
% \end{figure*}
This section first analyzes the limitations of existing work (Sec.\ref{subsec:limitation}). We especially focus on the currently best approach~\cite{bochen2024compilation}, providing concrete examples illustrating its limitations stemming from the separate addressing of various aspects of the problem mentioned in Sec.~\ref{sec:intro}. Building on this, 

illustrates the limitations of current work Enola (Sec.\ref{subsec:limitation}) using concrete examples. Building on this, we introduce the key motivations behind our solution, which addresses these shortcomings (Sec.\ref{subsec: our motivation}).
\todo{a little bit about why Enola? if not in intro, then here we must explain why Enola.}
\todo{existing compiler, why Enola}
\subsection{Analysis: Limitations of Enola}\label{subsec:limitation}
Enola’s framework decomposes the compilation problem into three sub-problems: (1) \emph{Scheduling}, which partitions CZ gates into \emph{stages} where gates within each stage can be executed in parallel; (2) \emph{Placement}, which determines an initial qubit layout that minimizes the total distance between interacting qubits; and (3) \emph{Routing}, which moves interacting qubits together while adhering to movement constraints. Enola uses efficient heuristics to solve each sub-problem, providing a solution for the overall problem. However, as mentioned in Sec.~\ref{sec:intro}, \todo{may move your insights from intro here or other fixing is needed} it suffers from two major drawbacks: (1) \emph{Suboptimal movement scheme}, and (2) \emph{Difficulty in storage zone integration}. We provide examples illustrating these issues respectively, and offer deeper insights into the underlying causes inherent in this solution, which finally motivates our solution. \todo{no storage zone}

\noindent\textbf{Example 1. Suboptimal Movement Scheme.} Enola’s movement scheme leads to unwanted qubit clustering when directly transitioning between layouts. For instance, Fig.\ref{fig:motivation}(a) shows the current qubit layout, where qubit pairs $(q_1,q_2)$, $(q_3,q_4)$, and $(q_5,q_6)$ are positioned close for CZ execution. In the next stage, we want to perform CZ gates on pairs $(q_2,q_3)$ and $(q_4,q_5)$. Enola would potentially move $q_2$ to $q_3$ and $q_4$ to $q_5$ for these interactions. However, this would create a cluster of $q_4,q_5,q_6$, preventing the desired CZ gate on $(q_4,q_5)$, as illustrated in Fig.\ref{fig:motivation}(b). To avoid this clustering issue, Enola reverts to the initial layout, where qubits are spatially separated (Fig.\ref{fig:motivation}(c)). From this intermediate layout, interacting qubits can be brought together without causing unwanted clustering (Fig.\ref{fig:motivation}(d)). However, constantly reverting to the initial layout introduces significant movement overhead, which could be minimized if we could directly transition between desired layouts for parallel CZ execution.


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{Figure/Motivation1012.pdf}
    \vspace{-6pt}
    \caption{Issue of qubit clustering. (a) . (b) .}
    \Description{Constraints}
    \label{fig:motivation} 
\end{figure}


\noindent\textbf{Example 2. Difficulty in Storage Zone Integration.} Enola’s framework requires reverting to the initial layout between stages. \todo{What we want to convey here is: 1. In their original paper, Enola did not distinguish between the compute and storage zones. 2. Simply extending their method does not work. I feel that the reviewer is not fully grasping the first point.} To integrate a storage zone, this initial layout would need to be placed entirely in the storage zone to avoid excitation errors, as shown in Fig.\ref{fig:motivation}(e). However, for each stage, interacting qubits would have to shuttle back and forth between the storage and computation zones in order to return to the initial layout. For example, to execute the two stages shown in Fig.\ref{fig:motivation}(a)(d), Enola would need to move the qubits as illustrated in Fig.~\ref{fig:motivation}(e)(f). This will result in significant inter-zone movement overhead.

These two examples prompt us to ask an important question: \emph{What is the fundamental reason behind these limitations?} Upon closer examination, we observe that the subproblems decomposed in Enola are inherently \emph{interdependent}, and optimizing them in isolation misses many opportunities for better solutions. For instance, separating qubit placement from gate routing prevents seamless transitions between layouts for CZ execution (Example 1). This creates a layout that is effectively semi-static, underutilizing the dynamic layout capabilities of NAQC and further hindering the efficient integration of the storage zone (Example 2). This observation leads us to the core motivation of our solution: adopt a \emph{holistic perspective}, recognizing and leveraging the interdependencies among various components and constraints to unlock new optimization possibilities.


\subsection{Motivation of~\frameworkname}{\label{subsec: our motivation}}

%First of all, we adopt transfer to dynamically change qubit layout without introducing more CZ gates, because the $0.1\%$ risk of atom loss due to transfer is cheaper than introducing extra CZ gate with infidelity $0.5\%$. 

Guided by the motivation outlined in Sec.~\ref{subsec:limitation}, we designed three key components that form the core of our solution. The workflow of~\frameworkname is presented in Fig.~\ref{fig:workflow}.

\noindent\textbf{1. Stage Scheduler.} We observed that the execution order of stages significantly impacts the cost of inter-zone communication. If the sets of interacting qubits between consecutive stages differ greatly, many qubits must shuttle between the storage and computation zones. To address this, we developed a \emph{stage scheduler} that not only partitions the input CZ gates into the minimal number of stages but also optimizes their order to minimize costly inter-zone movements (Sec.~\ref{sec:stage scheduler}).

\noindent\textbf{2. Continuous Router.} Enabling direct layout transitions requires careful handling of the interdependence between qubit positions and movement constraints. Our \emph{continuous router} addresses this by first identifying interacting qubit pairs at risk of clustering, then allocating them to the nearest available site to avoid clustering. Once all inter- and intra-zone movements are determined to enbale the desired CZ gates and qubit interchange between zones, they are grouped into Coll-Moves that comply with movement constraints.

\noindent\textbf{3. Coll-Move Scheduler.} We also observed that the execution order of Coll-Moves affects decoherence error. Scheduling the to-storage movements earlier and the to-compute movements later maximizes the time qubits remain in the storage zone, minimizing decoherence. Therefore, we developed a \emph{Coll-Move scheduler} that implements this strategy. Additionally, it leverages multiple AODs to execute several Coll-Moves in parallel, assigning moves to different AODs to minimize latency and boost system parallelism.

The technical details of these three components are presented in Sec.~\ref{sec:stage scheduler}, Sec.~\ref{sec:conti router}, and Sec.~\ref{sec:Move scheduler}, respectively.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{Figure/Workflow.pdf}
    \vspace{-6pt}
    \caption{Workflow of~\frameworkname.}
    \Description{Workflow}
    \label{fig:workflow} 
\end{figure}


==> TexFile/05_Overview.tex <==
\section{Overview}\label{sec:overview}
This section presents an overview of~\frameworkname's workflow based on three core components we developed: (1) \emph{Stage scheduler}, (2) \emph{Continuous router}, (3) \emph{Coll-Move scheduler}, as presented in Fig.~\ref{fig:workflow}.

\noindent\textbf{Step 1. Stage Scheduler. }
\subsection{Preparation}\label{subsec:preparation}
The input benchmark circuits are synthesized into alternating layers of single-qubit gates and CZ gate blocks. Since the single-qubit gate layers can be executed in parallel using (see Sec.~\ref{sec:background}), we focus on optimizing within each CZ block.

\noindent\textbf{Stage Partition.} Within a CZ block, all CZ gates commute, allowing for arbitrary execution order. CZ gates acting on distinct qubits can be executed in parallel once the qubits are within the Rydberg radius. We define such parallel groups as \emph{stages} and use an edge coloring algorithm~\cite{misra1992constructive, bochen2024compilation} to partition CZ blocks into stages with the number of stages minimized.

\noindent\textbf{Initial Layout.} Prior to computation, qubits are placed in the storage zone following the initial layout used in~\cite{bochen2024compilation}, which heuristically minimizes movement distance between interacting qubit pairs and facilitates subsequent CZ gates.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{Figure/Workflow1013.pdf}
    \vspace{-6pt}
    \caption{Workflow of~\frameworkname.}
    \Description{Workflow}
    \label{fig:workflow} 
\end{figure}

\subsection{\frameworkname's Workflow}

After the preparation stage, the compilation problem reduces to optimizing the CZ stages. \frameworkname~consists of the following four steps, as Fig.~\ref{fig:workflow} shows.

\noindent\textbf{Inter-Stage Scheduler.} The \emph{inter-stage scheduler} determines the execution order of stages to minimize qubit interchange between zones, thereby reducing inter-zone movement overhead. The key idea is to begin with the stage involving the fewest qubits and then iteratively select the next stage with the smallest difference in the set of interacting qubits.

\noindent\textbf{Continuous Router.} Given the order of stage execution, the continuous router dynamically adjusts the qubit layout without reverting to previous layouts. This approach significantly reduces total movement time, the number of transfers, and ultimately decoherence error. The core idea is to assign qubits their next movement based on the upcoming CZ gates, determining both inter-zone and intra-entangling zone movements while avoiding potential qubit clustering. These individual qubit movements are then grouped into collective movements that comply with AOD constraints.

\noindent\textbf{Intra-Stage Scheduler.} The \emph{intra-stage scheduler} optimizes the order of collective movements within each stage to maximize the time qubits remain in the storage zone. This is done by prioritizing the entangle-to-storage moves and delaying the storage-to-entangle moves.

\noindent\textbf{Multi-AOD Scheduler.} Finally, the ordered collective movements are distributed across multiple AOD frames to increase parallelism and reduce movement time. The key idea is to balance the total movement time across all AODs within a stage, minimizing overall latency.

The following sections (Sec.\ref{sec:conti router},\ref{sec:stage scheduler},~\ref{sec:multi-AOD scheduler}) provide detailed designs of these components.



==> TexFile/07_Eval_01.tex <==
\begin{table}[h]
    \centering
      \caption{Benchmarks.}
      % \vspace{-5pt}
      
    \resizebox{0.48\textwidth}{!}{
        \renewcommand*{\arraystretch}{1}
        \begin{footnotesize}
        \begin{tabular}{|p{1.7cm}|p{1.5cm}|p{2.0cm}|p{1.4cm}|p{1.6cm}|}  \hline
        Name & \#Qubits & Compute Zone Size (${\mu m}^2$) & Inter Zone Size (${\mu m}^2$) & Storage Zone Size (${\mu m}^2$)\\ 
        \hline
        \multirow{6}{*}{QAOA-regular3}  
                     & 30 & 90 x 90 & 90 x 30 & 90 x 180\\ 
        \cline{2-5}  & 40 & 105 x 105 & 105 x 30 & 105 x 210\\
        \cline{2-5}  & 50 & 120 x 120 & 120 x 30 & 120 x 240\\
        \cline{2-5}  & 60 & 120 x 120 & 120 x 30 & 120 x 240\\
        \cline{2-5}  & 80 & 135 x 135 & 135 x 30 & 135 x 270\\
        \cline{2-5}  & 100 & 150 x 150 & 150 x 30 & 150 x 300\\
        \hline
        \multirow{5}{*}{QAOA-regular4}  
                     & 30 & 90 x 90 & 90 x 30 & 90 x 180\\ 
        \cline{2-5}  & 40 & 105 x 105 & 105 x 30 & 105 x 210\\
        \cline{2-5}  & 50 & 120 x 120 & 120 x 30 & 120 x 240\\
        \cline{2-5}  & 60 & 120 x 120 & 120 x 30 & 120 x 240\\
        \cline{2-5}  & 80 & 135 x 135 & 135 x 30 & 135 x 270\\
        \hline
        \multirow{2}{*}{QAOA-random}  
                     & 20 & 75 x 75 & 75 x 30 & 75 x 150\\ 
        \cline{2-5}  & 30 & 90 x 90 & 90 x 30 & 90 x 180\\
        \hline
        \multirow{2}{*}{QFT}  
                     & 18 & 75 x 75 & 75 x 30 & 75 x 150\\ 
        \cline{2-5}  & 29 & 90 x 90 & 90 x 30 & 90 x 180\\ 
        \hline
        \multirow{3}{*}{BV}  
                     & 14 & 60 x 60 & 60 x 30 & 60 x 120\\ 
        \cline{2-5}  & 50 & 120 x 120 & 120 x 30 & 120 x 240\\
        \cline{2-5}  & 70 & 120 x 120 & 120 x 30 & 120 x 240\\
        \hline
        \multirow{2}{*}{VQE}  
                     & 30 & 90 x 90 & 90 x 30 & 90 x 180\\ 
        \cline{2-5}  & 50 & 120 x 120 & 120 x 30 & 120 x 240\\
        \hline
        \multirow{3}{*}{QSIM-rand-0.3}  
                     & 10 & 60 x 60 & 60 x 30 & 60 x 120\\ 
        \cline{2-5}  & 20 & 75 x 75 & 75 x 30 & 75 x 150\\ 
        \cline{2-5}  & 40 & 105 x 105 & 105 x 30 & 105 x 210\\
        \hline
        % \cline{2-4} & 25 & 5x5 & 60x60 \\
        % % \cline{2-4} & 36 & 6x6 & 60x60 \\
        % \hline
        %  \multirow{4}{*}{0.75}  & 4 & 2x2 & 48x48\\
        % \cline{2-4}  & 25 & 5x5 & 120x120 \\
        % \cline{2-4} & 64 & 8x8 & 192x192 \\
        % \cline{2-4} & 100 & 10x10 & 240x240 \\
        % \hline
         
         
        \end{tabular}
        \end{footnotesize}
    }
 % \vspace{-10pt}
    \label{tab:benchmark}
\end{table}

\section{Evaluation}\label{sec:eval}
\begin{table*}[tp]
    \centering
    \caption{The results of our compiler and its relative performance to the baseline. Each benchmark-$n$' corresponds to an $n$-qubit circuit in the circuit model.}
    % , evaluated on a entangling zone area of size $15\times\lceil\sqrt{n}\rceil\times15\times\lceil\sqrt{n}\rceil\ {\mu m}^2$, inter zone area of size $30\times15\times\lceil\sqrt{n}\rceil\ {\mu m}^2$ and a storage zone area of size $2 \times 15 \times\lceil\sqrt{n}\rceil\times15\times\lceil\sqrt{n}\rceil\ {\mu m}^2$.
  %  The name column are acronyms of test programs in Table~\ref{tab:benchmark}.}
   \resizebox{\textwidth}{!}{
        \renewcommand*{\arraystretch}{1.3}
        \begin{large}
            
            \begin{tabular}{|p{3.2cm}|| p{1.6cm}|p{2.3cm}|p{2.3cm}|p{1.7cm}||p{2.1cm}|p{2.3cm}|p{2.3cm}|p{2.1cm}||p{2.3cm}|p{2.1cm}|p{2.3cm}|}
        
        \hline
        Benchmark - \#Qubit & Enola Fidelity& Our Fidelity (non-storage) & Our Fidelity (with-storage) & Fidelity \ \ Improv.  & Enola $T_{exe}(\mu s)$ & Our $T_{exe}(\mu s)$ (non-storage) & Our $T_{exe}(\mu s)$ (with-storage) & $T_{exe}$ Improv. & Enola $T_{comp}(s)$ & Our $T_{comp}(s)$ & $T_{comp}$ Improv.\\
        \hline
        \hline

        QAOA-regular3-30 & 0.48 & 0.64 & 0.68 & 1.41 & 13,198.04 & 4,680.72 & 6,116.19 & 2.82 & 128.32 & 41.33 & 3.10\\
        \hline
        QAOA-regular3-40 & 0.34 & 0.53 & 0.57 & 1.67 & 17,249.38 & 5,601.12 & 8,998.75 & 3.08 & 144.70 & 41.50 & 3.49\\
        \hline
        QAOA-regular3-50 & 0.23 & 0.43 & 0.49 & 2.12 & 21,087.88 & 7,135.26 & 9,582.99 & 2.96 & 142.30 & 41.49 & 3.43\\
        \hline
        QAOA-regular3-60 & 0.14 & 0.35 & 0.39 & 2.70 & 25,449.73 & 8,134.16 & 12,440.46 & 3.13 & 140.64 & 44.62 & 3.15\\
        \hline
        QAOA-regular3-80 & 0.05 & 0.22 & 0.24 & 4.90 & 33,553.14 & 10,490.10 & 17,746.76 & 3.2 & 145.91 & 45.38 & 3.22\\
        \hline
        QAOA-regular3-100 & 0.01 & 0.10 & 0.14 & 12.82 & 44,038.42 & 16,122.96 & 21,710.11 & 2.73 & 167.22 & 45.64 & 3.66\\
        \hline
        QAOA-regular4-30 & 0.40 & 0.56 & 0.56 & 1.42 & 16,450.23 & 6,056.05 & 12,127.03 & 2.72 & 256.88 & 65.33 & 3.93\\
        \hline
        QAOA-regular4-40 & 0.24 & 0.45 & 0.42 & 1.72 & 23,365.45 & 7,394.03 & 17,608.55 & 3.16 & 266.53 & 66.07 & 4.03\\
        \hline
        QAOA-regular4-50 & 0.14 & 0.34 & 0.31 & 2.27 & 30,079.41 & 9,928.27 & 20,013.50 & 3.03 & 253.94 & 63.34 & 4.01\\
        \hline
        QAOA-regular4-60 & 0.07 & 0.26 & 0.23 & 3.22 & 36,332.16 & 11,306.93 & 22,594.20 & 3.21 & 278.18 & 68.89 & 4.04\\
        \hline
        QAOA-regular4-80 & 0.01 & 0.10 & 0.09 & 6.06 & 49,182.73 & 19,631.36 & 32,934.94 & 2.51 & 291.68 & 72.17 & 4.04\\
        \hline
        QAOA-random-20 & 0.23 & 0.39 & 0.47 & 2.02 & 32,768.58 & 11,782.99 & 16,845.33 & 2.78 & 960.37 & 136.03 & 7.06\\
        \hline
        QAOA-random-30 & 0.03 & 0.11 & 0.16 & 5.85 & 68,113.52 & 25,391.69 & 38,051.69 & 2.68 & 1791.66 & 193.28 & 9.27\\
        \hline
        QFT-18 & $8.95 \times 10^{-4}$  & $4.87 \times 10^{-3}$ & 0.05 & 60.30 & 108,173.62 & 36,810.15 & 107,637.68 & 2.94 & 10917.80 & 347.47 & 31.42\\
        \hline
        QFT-29 & $7.12 \times 10^{-9}$ & $9.99 \times 10^{-7}$ & $5.78 \times 10^{-4}$ & 81,151.50 & 239,150.00 & 89,670.26 & 237,315.37 & 2.67 & 24116.00 & 511.97 & 47.10\\
        \hline
        BV-14 & 0.57 & 0.60 & 0.91 & 1.58 & 5,583.98 & 3,034.20 & 5,282.11 & 1.84 & 669.48 & 28.79 & 23.26\\
        \hline
        BV-50 & 0.04 & 0.05 & 0.84 & 20.20 & 10,118.96 & 5,631.26 & 9,255.85 & 1.8 & 1710.91 & 17.95 & 95.32\\
        \hline
        BV-70 & $6.92 \times 10^{-4}$ & $1.05 \times 10^{-3}$ & 0.75 & 1,090.36 & 17,620.11 & 10,277.27 & 15,942.37 & 1.71 & 4334.5 & 20.30 & 213.55\\
        \hline
        VQE-30 & 0.71 & 0.81 & 0.79 & 1.12 & 5,436.18 & 1,688.03 & 2,981.71 & 3.22 & 57.62 & 29.68 & 1.94\\
        \hline
        VQE-50 & 0.48 & 0.67 & 0.63 & 1.32 & 10,196.50 & 2,946.26 & 5,354.37 & 3.46 & 56.58 & 29.86 & 1.89\\
        \hline
        QSIM-rand-10 & 0.51 & 0.60 & 0.74 & 1.45 & 13,353.05 & 4,886.36 & 9,713.39 & 2.73 & 760.19 & 76.01 & 10.00\\
        \hline
        QSIM-rand-20 & 0.05 & 0.08 & 0.42 & 9.02 & 37,796.35 & 16,636.02 & 35,550.68 & 2.27 & 5740.76 & 107.03 & 53.64\\
        \hline
        QSIM-rand-40 & $3.94 \times 10^{-6}$ &  $2.39 \times 10^{-5}$ & 0.14 & 35,519.88 & 93,062.71 & 45,424.55 & 89,418.81 & 2.05 & 8283.45 & 127.95 & 64.74\\
        \hline
    \end{tabular}
    \end{large}
    }
    \label{tab:main_table}
\end{table*}

\subsection{Experiment Setup}


\vspace{0.3em}
\noindent \textbf{Hardware setting.}
%In our default setup, adjacent qubits are spaced \(15 \, \mu m\) apart, with a distance of \(30 \, \mu m\) between the entangling zone and the storage zone. Both fidelity and execution duration values are aligned with the latest experimental benchmarks, as shown in Table \ref{tab:NA hardware parameter}.
As outlined in Table \ref{tab:NA hardware parameter}, our hardware configuration follows the latest experimental data. In the default setup, adjacent qubits are spaced \(15 \, \mu m\) apart, with a distance of \(30 \, \mu m\) between the compute zone and the storage zone. Both the fidelity and execution times of entangling operations align with the most recent experimental settings.


\vspace{0.3em}
\noindent \textbf{Metrics.} We evaluate the compiler's performance using three metrics. The first metric, defined as \emph{Fidelity},  refers to the overall circuit fidelity, as described in detail in Section \ref{sec:background}. The second metric is the execution time, denoted as \emph{$T_{exe}$}, which accounts for the total time needed for executing single-qubit and two-qubit gates, as well as qubit transfer and movement. The third metric is the compilation time, denoted as $T_{comp}$, which represents the duration taken to transform the high-level quantum program into a low-level implementation suitable for NAQC, including optimization and scheduling processes.


\vspace{0.3em}
\noindent \textbf{Baselines.} 
We focus primarily on comparing PowerMove with Enola~\cite{bochen2024compilation}, the state-of-the-art neutral atom compiler. Enola has demonstrated superior performance over previous neutral atom compilers, particularly for large-scale programs, with two-qubit fidelity 779 times higher than Atomique~\cite{wang2024atomique} and 5806 times higher than Q-Pilot~\cite{wang2023q}. Our evaluation corroborates Enola's claims, which is why we focus on this comparison for a more concise and relevant analysis. Earlier compilers~\cite{tan2022qubit, tan2024compiling, bochen2024compilation} did not leverage the unique hardware features of neutral atom systems, resulting in significantly worse performance. A direct comparison with them would not be fair or meaningful in this context.
%To highlight the advantages of PowerMove, we compare it with the latest neutral atom compiler framework, Enola~\cite{bochen2024compilation}, which significantly outperforms previous neutral atom compilers. Specifically, for large-scale programs, its two-qubit gate fidelity is 779 times higher than Atomique~\cite{wang2024atomique} and 5806 times higher than Q-Pilot~\cite{wang2023q}. We also conducted experiments comparing PowerMove with earlier compilers, and our results are consistent with these performance trends.


\vspace{0.3em}
\noindent \textbf{Benchmarks.}
We evaluate performance using a variety of benchmark programs, including Quantum Approximate Optimization Algorithm (QAOA), Quantum Simulation (QSim), Quantum Fourier Transform (QFT), Bernstein-Vazirani (BV) algorithm, and Variational Quantum Eigensolver (VQE). For QAOA, we use two circuit types: one with randomly placed ZZ gates between qubit pairs (50\% probability), and another based on regular graphs, where ZZ gates apply only to qubits connected by graph edges. QSim circuits are randomly generated with a 0.3 probability for a non-identity Pauli operator on each qubit, with ten Pauli strings per circuit. BV circuits use randomly generated secret strings, with an even distribution of 0s and 1s. For VQE, we follow the standard full-entanglement ansatz.
% We select a set of benchmark programs including Quantum Approximate Optimization Algorithm (QAOA), Quantum Simulation (QSim), Quantum Fourier transform (QFT), Bernstein-Vazirani (BV) algorithm and Variational Quantum Eigensolver (VQE). We use two types of QAOA circuits. The first type is constructed by randomly placing ZZ gates between pairs of qubits with a 50\% probability. The second type is generated based on regular graphs, where ZZ interactions are applied only to qubit pairs connected by edges in the graph. QSim circuits are randomly generated with a probability of 0.3 for a qubit to exhibit a non-I Pauli operator, and each circuit comprises ten Pauli strings. For BV, we select the secret strings randomly, with approximately half of the digits being 0 and half being 1.  For VQE, we follow the commonly used full-entanglement ansatz, which proves to be an expressive ansatz.  

For an \(n\)-qubit program, our default configuration features a \(\lceil\sqrt{n}\rceil \times \lceil\sqrt{n}\rceil\) topology, allowing one AOD transfer at a time. Additionally, the storage zone is configured as a \(2 \times \lceil\sqrt{n}\rceil \times \lceil\sqrt{n}\rceil\) topology. The hardware dimensions are as follows: the compute zone measures \(15 \times \lceil\sqrt{n}\rceil \times 15 \times \lceil\sqrt{n}\rceil \, {\mu m}^2\), the inter-zone size is \(30 \times 15 \times \lceil\sqrt{n}\rceil \, {\mu m}^2\), and the storage zone measures \(2 \times 15 \times \lceil\sqrt{n}\rceil \times 15 \times \lceil\sqrt{n}\rceil \, {\mu m}^2\). In Table \ref{tab:benchmark}, we present the benchmarks along with the number of qubits in their circuit representation and the size of their moving area.

\input{TexFile/11_tables}

% To assess compiler performance, we utilize
% three benchmark categories: algorithmic (generic), quantum
% simulation (QSim), and Quantum Approximate Optimization
% Algorithm (QAOA). Their characteristics are detailed in Table II. The metric “Degree per Q” represents the average
% count of unique qubits that interact with a given qubit.
% Algorithmic circuits are sourced from SupermarQ [81] and
% QASMBench [47]. QSim circuits are randomly generated with
% a probability of 0.5 for a qubit to exhibit a non-I Pauli
% operator, and each circuit comprises ten Pauli strings. For
% molecular Hamiltonians, we consider H2 and LiH. QAOA
% circuits are constructed by randomly placing ZZ gates between
% all pairs of qubits with a probability of 0.5. In addition,
% QAOA circuits based on regular graphs are generated, in which
% ZZ interactions are placed to qubit pairs with an edge in
% the regular graph. These benchmarks span a broad spectrum
% featuring a variety number of qubits and circuit depth.

% \noindent\textbf{Fidelity Calculation.}
% We omit the fidelity term associated with the single-qubit gates because they are equal across the comparison.

\subsection{Main Results}\label{subsection: main results}
% Table~\ref{tab:main_table} presents a comparison between our framework and Enola. The results show that our approach significantly improves both circuit fidelity and execution time. 

% For large-scale programs, it achieves an overall fidelity improvement of several orders of magnitude compared to Enola. Additionally, it accelerates the execution time of compiled programs by 1.71x to 3.46x, as shown in the \emph{Fidelity Improv.} and \emph{$T_{exe}$ Improv.} columns. Fidelity improvement grows exponentially as the number of qubits increases, while the enhancement in program execution time remains stable.

% Specifically, we divide our results into two cases: the non-storage (without zoned architecture) case and the with-storage (with zoned architecture) case. The results show that the storage zone provides a much more significant advantage in large-scale programs and benchmarks like QAOA-random, QFT, BV, and QSIM-rand. This is because the zoned architecture is primarily designed to mitigate qubit excitation errors during Rydberg light execution, and the occurrence of these errors increases with the number of Rydberg light executions, which is directly correlated to program size and the structure of the benchmark circuits. Meanwhile, utilizing the zoned architecture introduces additional move-in and move-out operations between the entangling zone and the storage zone, resulting in a slight overhead in the execution time, as shown in the \emph{Our $T_{exe}(\mu s)$ (with-storage)} column, while the execution time remains faster than in the Enola case.\\


In this subsection, we compare our compiler with Enola in terms of fidelity and execution time across two scenarios: the non-storage case, where continuous routing is applied, and the with-storage case, which incorporates the zoned architecture for enhanced performance. We also evaluate the compilation time for both scenarios.
%reporting the average across both scenarios.

\vspace{0.3em}
\noindent \textbf{Overall Performance.}
 % As detailed in the \emph{Fidelity Improv.} and \emph{$T_{exe}$ Improv.} columns in Fig. \ref{tab:main_table}, our approach achieves fidelity enhancements that are several orders of magnitude better than Enola for large-scale programs.
 As detailed in the \emph{Fidelity Improv.} and \emph{$T_{exe}$ Improv.} columns in Fig. \ref{tab:main_table}, our framework consistently outperforms the Enola framework, which only maintains reasonable fidelity for small-scale programs. In contrast, our approach enables large-scale programs to sustain high fidelity, particularly in the QSIM-rand and BV benchmarks. For instance, in the 70-qubit BV scenario, while Enola reports a low fidelity of \(6.92 \times 10^{-4}\), our method achieves a fidelity of \(0.75\). This substantial improvement demonstrates our framework's ability to run much larger programs with high accuracy in the NISQ era.
 Additionally, the execution time of compiled programs is sped up by 1.71x to 3.46x. Notably, fidelity improvements grow exponentially with the number of qubits. Meanwhile, the execution time improvements remain stable or show slight increases as the qubit count rises.

\vspace{0.3em}
\noindent \textbf{Continuous Routing Improvement.}
% In the non-storage case, applying the continuous routing algorithm yields an average fidelity improvement of up to 8.90x, as shown in the \emph{Our Fidelity (non-storage)} column, alongside a significant reduction in execution time, as seen in the \emph{Our $T_{exe}(\mu s)$ (non-storage)} column. 
In the non-storage case, applying the continuous routing algorithm yields an average fidelity improvement of up to 8.90x, as shown in the \emph{Our Fidelity (non-storage)} column, alongside a significant reduction in execution time, as seen in the \emph{Our $T_{exe}(\mu s)$ (non-storage)} column. Our optimization origins from the continuous router, which reduces movement and transfer counts by approximately half. Since decoherence errors grow exponentially with decoherence time, the optimization effects are particularly pronounced in large-scale programs and the benchmarks for QAOA-regular3, QAOA-regular4, QAOA-random, and QFT, as these benchmarks inherently have longer decoherence times.

% \todo{This improvement is particularly pronounced in large-scale programs and in the benchmarks for QAOA-regular3, QAOA-regular4, QAOA-random, and QFT, as both scenarios lead to more decoherence errors and greater optimization potential. In large-scale programs, the increase in program size results in more CZ interactions, which in turn leads to greater qubit movement and longer decoherence times, resulting in more decoherence errors. In the other case, the unique structures of the above benchmarks result in each CZ block containing more CZ gates, leading to more interactions within each stage, longer decoherence times, and a higher proportion of decoherence errors relative to the overall circuit errors.}

\vspace{0.3em}
\noindent \textbf{With-Storage Improvement.}
In the with-storage case, the zoned architecture offers a notable advantage in fidelity, particularly for large-scale benchmarks such as QAOA-random, QFT, BV, and QSim-rand, boosting fidelity improvements to as much as $8.15 \times 10^4$x. This benefit arises because the zoned architecture is specifically designed to mitigate qubit excitation errors during Rydberg light operations, which increase in frequency with the number of operations as the program size and circuit complexity grow. 


However, the zoned architecture introduces a minor overhead in execution time due to the additional move-in and move-out operations between the compute and storage zones. This slight loss in time efficiency is worthwhile, as improving program fidelity is crucial in the NISQ era. This trade-off results in an average fidelity improvement of 313.86x compared to the non-storage case, making it a valuable gain. Additionally, as shown in the \emph{Our $T_{exe}(\mu s)$ (with-storage)} column, our execution time remains faster than that of Enola. This is largely due to the significant execution time improvements provided by the continuous routing algorithm.

\noindent \textbf{Compilation Time.}
As detailed in the $T_{comp}$ Improv. column of Table \ref{tab:main_table}, our framework achieves remarkable compilation time improvements of up to 213.5 times compared to Enola. This enhancement grows with the size of the program, demonstrating its effectiveness in handling larger-scale computations. The challenges of compilation optimization within the NAQC NISQ paradigm are significant, as many of these problems are NP-hard.  Enola, for instance, employs maximum independent set (MIS) solvers, which can lead to prolonged compilation times. In contrast, our approach utilizes a near-linear heuristic algorithm, significantly reducing the compilation time while effectively managing the complexities of these NP-hard tasks.

% Our framework achieves remarkable compilation time improvements of up to 213.5 times compared to Enola, as detailed in the $T_{comp}$ Improv. column of Table \ref{tab:main_table}. This enhancement grows with the size of the program, demonstrating its effectiveness in handling larger-scale computations.

% The challenges of compilation optimization within the NAQC NISQ paradigm are significant, as many of these problems are NP-hard. Existing compilers, such as Enola, often rely on computationally intensive solvers like maximum independent set (MIS) algorithms, which can lead to prolonged compilation times.

% To address these issues, we developed a near-linear heuristic algorithm for collective movement grouping. This approach not only expedites the compilation process but also effectively manages the complexities inherent in these NP-hard optimization problems.

% \todo{?}

% Specifically, the experiments show that Enola can work only in the region of small programs and high fusion success probabilities. When the fusion success probability decreases to a practical value around 0.75, it takes more than $10^6$ RSLs to even execute the 4-qubit benckmarks. This implies OneQ's non-scalability due to its lack of capability in systematically handling the randomness of fusion failure. 
% In contrast, our framework can work well with a practical success probability, demonstrating an increasing outperformance over OneQ as the programs scale up.
% \subsection{Scalability}\label{subsec:Scalability}

% In this section, we demonstrate the scalability of our compiler framework by focusing on three key aspects: fidelity, execution time, and compilation time. In NISQ era, fidelity is the most crucial because it determines the size of quantum programs we can execute while still achieving accurate results. Higher fidelity allows us to run larger programs with reliable outcomes. Execution time is critical, as quantum coherence is limited. Shorter execution times allow for running larger programs within this limited period. Additionally, reducing execution time helps minimize decoherence errors, improving the likelihood of successful program execution. Lastly, compilation time plays a significant role in scalability. Many existing compilers, such as Enola, face inefficiencies when handling large programs, with excessively long compilation times—for instance, taking 6.70 hours to compile a 29-qubit QFT, which is impractical.  Our framework addresses these challenges, making it highly scalable for larger quantum applications while maintaining both accuracy and time efficiency.

% \vspace{0.3em}
% \noindent \textbf{Fidelity.}
% As shown in Fig. \ref{fig:fidelity ablation}, our framework consistently outperforms the Enola framework, which only maintains reasonable fidelity for small-scale programs. In contrast, our approach enables large-scale programs to sustain high fidelity, particularly in the QSIM-rand and BV benchmarks. For instance, in the 70-qubit BV scenario, while Enola reports a low fidelity of \(6.92 \times 10^{-4}\), our method achieves a fidelity of \(0.75\). This substantial improvement demonstrates our framework's ability to run much larger programs with high accuracy in the NISQ era.
% \todo{an ending sentence.}
% As illustrated in Fig. \ref{fig:fidelity ablation}, our framework consistently outperforms the Enola framework, which only maintains reasonable fidelity for small-scale programs. In contrast, our approach enables high fidelity even for large-scale programs, particularly evident in the QSIM-rand and BV benchmarks. For example, in the 70-qubit BV case, while Enola achieves a low fidelity of \(6.92 \times 10^{-4}\), our method reaches a significantly higher fidelity of \(0.75\). This substantial improvement demonstrates our framework's ability to run much larger programs with high accuracy in the NISQ era, showcasing its scalability and effectiveness for complex quantum tasks.

% \subsection{Time Efficiency}\label{subsec:Time Efficiency}
% In this subsection, we emphasize improvements in time efficiency. First, we leverage multiple AODs to accelerate execution time, enabling the execution of larger programs within the constraints of limited coherence time. Additionally, we compare our compilation time with Enola's across various benchmarks with increasing qubit counts, demonstrating our enhanced scalability in compilation efficiency.



% \todo{I feel that the multi-AOD setting is worthy to be mentioned earlier, instead of being briefly mentioned under execution time.}
% As shown in Table \ref{tab:main_table}, our framework achieves stable or slightly increased execution time improvements across various benchmarks as the number of qubits grows. 

% \todo{enrich this part.}
% As demonstrated in Table \ref{tab:main_table}, our framework consistently achieves stable or even slightly improved execution times across various benchmarks as the number of qubits increases. A key factor in this improvement is the use of multiple Acousto-Optic Deflectors (AODs), which significantly accelerate execution by distributing previously conflicting qubit movement operations across different AODs. This distribution increases the parallelism of collective movements, as illustrated in Fig. \ref{fig:multi_aod}, leading to a substantial reduction in the execution time of compiled programs. Furthermore, the overall circuit fidelity remains stable or improves slightly, as reduced decoherence times enhance the decoherence fidelity of the system.





% \todo{My thought is that among paragraphs for fidelity, execution time and compilation time, the first doesn't provide much information and can be combined with previous discussion; the multi-AOD doesn't really count as scalability but is worthy for being emphasized earlier; the faster compilation for scalability can be discussed separately. If you think only discussing compilation time is not enough, you can also analyze why our compiler should also work for larger scale like beyond 100 qubits.}

\subsection{Ablation Study}\label{subsec:Ablation}

In this section, we analyze the impact of continuous routing and zoned architecture on different components of fidelity as circuit scales increase across various benchmark circuits. As illustrated in Fig. \ref{fig:fidelity ablation}, the green section represents two-qubit infidelity, the blue section corresponds to excitation error, the purple section indicates qubit transfer infidelity, and the yellow section highlights the decoherence error. Our framework primarily targets the elimination of the last three fidelity components: excitation error, qubit transfer infidelity, and decoherence error. We also evaluate the acceleration achieved through multi-AOD configurations and assess their impact on fidelity across different benchmarks.


% \todo{The following three paragraphs may need to be rephrased. The Fig. are great, but the texts don't look good enough.}
\vspace{0.3em}
\noindent \textbf{Excitation Error Reduction.}
% As shown in Fig. \ref{fig:fidelity ablation}, our framework exhibits a significantly less pronounced decline in fidelity with increasing qubit count compared to Enola, particularly in the QSIM-rand and BV benchmarks, as shown in Fig. \ref{fig:fidelity ablation}(b) and \ref{fig:fidelity ablation}(e). This unique improvement is attributed to the structure of these benchmarks, which contains a higher number of dependent CZ blocks, each with relatively few CZ gates. This leads to significantly more Rydberg light execution stages and a relatively shorter overall movement distance in the QSIM-rand and BV cases. In the Enola framework, this configuration leads to a significant occurrence of excitation errors, whereas our zoned architecture effectively mitigates these errors. This substantial optimization is evident in the with-storage graphs in Fig. \ref{fig:fidelity ablation}(b) and \ref{fig:fidelity ablation}(e).
As shown in the blue part of Fig. \ref{fig:fidelity ablation}, our framework demonstrates an exponential reduction in excitation errors with increasing qubit count compared to Enola, particularly in the QSIM-rand and BV benchmarks, as illustrated in Fig. \ref{fig:fidelity ablation}(b) and \ref{fig:fidelity ablation}(e). This improvement is primarily attributed to our zoned architecture, which effectively mitigates excitation rates. In QSIM-rand and BV benchmarks, the structure comprises numerous dependent CZ blocks, each containing relatively few CZ gates. This configuration leads to a higher number of Rydberg execution stages that can contribute to excitation errors. Consequently, the optimization of excitation errors in our framework is particularly pronounced in these benchmarks. This substantial enhancement is clearly reflected in the with-storage graphs in Fig. \ref{fig:fidelity ablation}(b) and \ref{fig:fidelity ablation}(e).


% \todo{a bit influent}





\vspace{0.3em}
\noindent \textbf{Decoherence Fidelity Improvement.} 
% Similarly, significant reductions in decoherence errors are observed in the QAOA, QFT, and VQE benchmarks, as shown in Fig. \ref{fig:fidelity ablation}(a), (c), and (d). As with qubit transfer, the structure of these benchmarks involves a higher number of move operations within each stage, providing more opportunities to optimize decoherence time and, consequently, improve decoherence fidelity.
As exhibited in the yellow part of Fig. \ref{fig:fidelity ablation}, significant reductions in decoherence errors are also observed, particularly in the QAOA-regular3, QFT, and VQE benchmarks. This improvement is primarily due to our continuous routing algorithm, which minimizes redundant movement operations, thereby reducing decoherence time and, consequently, lowering decoherence errors. In the QAOA-regular3, QFT, and VQE benchmarks, the density and frequency of movement operations are relatively higher, which provides greater optimization potential for reducing decoherence errors.



\vspace{0.3em}
\noindent \textbf{Transfer Fidelity Enhancement.} 
% As shown in Fig. \ref{fig:fidelity ablation}, the improvement in transfer fidelity is more significant in the QAOA, QFT, and VQE benchmarks, illustrated in Fig. \ref{fig:fidelity ablation}(a), (c), and (d). This is because these benchmarks feature fewer dependent CZ blocks, but each block contains a higher number of CZ gates, leading to more frequent transfer operations within each stage. This configuration provides a larger optimization space for reducing transfer infidelity.
As shown in the purple part of Fig. 6, there is also a noticeable reduction in transfer error, although the improvement in transfer fidelity is comparatively less pronounced compared to other fidelity metrics. This is primarily because the fidelity of individual transfer operations is already very high, at 99.9\%. The optimization of transfer fidelity is relatively evident in the QAOA, QFT, and VQE benchmarks. These benchmarks involve denser movement operations within each Rydberg stage, resulting in more frequent transfer operations. This configuration creates a larger optimization space for enhancing transfer fidelity.
% Additionally, \todo{?} we can leverage multiple AODs to accelerate execution, as illustrated in Fig. \ref{fig:multi_aod}, which significantly accelerate execution by distributing previously conflicting qubit movement operations across different AODs. This distribution increases the parallelism of Coll-Moves, leading to a substantial reduction in the execution time of compiled programs. Importantly, overall circuit fidelity remains stable or improves slightly, as the decrease in decoherence time enhances decoherence fidelity. \todo{why?}

\vspace{0.3em}
\noindent \textbf{Multiple AODs.}
Additionally, when we have less constrained hardware resources to utilize multiple AODs, we can leverage them to parallelize movement and transfer operations, which would otherwise be limited by the constraints of a single AOD. As illustrated in Fig. \ref{fig:multi_aod}, even with a limited number of AODs, we achieve noticeable acceleration, demonstrating that substantial speed improvements can be realized without the need for excessive hardware resources. Notably, our fidelity optimization is more evident in benchmarks with higher decoherence errors, as shown in the fidelity section of Fig.~\ref{fig:multi_aod}, represented by the blue, green, and yellow bars corresponding to the QAOA-regular3, QSIM-rand-0.3, and VQE benchmarks, respectively. This improvement is due to the increased parallelism afforded by multi-AOD configurations, which effectively reduces decoherence time and, consequently, minimizes decoherence errors.


% \begin{Fig.*}[tp]
%         % \hspace{-1pt}
%         \centering
%         \includegraphics[width=\linewidth]{Fig./qaoa-regular3.pdf}
%         % \vspace{-5pt}
%         \textbf{(a) QAOA-regular3} 
%         % \todo{This caption should be closer to the row above than the row below}}
%         % \vspace{-5pt}
%         \centering
%         \includegraphics[width=\linewidth]{Fig./qsim_rand_0.3.pdf}
%         \textbf{(b) QSIM-rand-0.3}
%         \centering
%         \includegraphics[width=\linewidth]{Fig./qft.pdf}
%         \textbf{(c) QFT}
%         \includegraphics[width=\linewidth]{Fig./vqe.pdf}
%         \textbf{(d) VQE}
%         \includegraphics[width=\linewidth]{Fig./bv.pdf}
%         \textbf{(e) BV}
%         \caption{Effects of the continuous routing algorithm and the introduction of zoned architecture on QAOA-regular3, QSIM-rand-0.3, QFT, VQE, and BV benchmark circuits. This study evaluates various numbers of qubits and focuses on four key components of overall circuit fidelity.}

%         \label{fig:fidelity ablation}
% \end{Fig.*}

\begin{figure*}[tp]
    % \centering
    % \includegraphics[width=\linewidth]{Fig./blank.pdf}
    % \centering
    % \vspace{-1pt}
    \includegraphics[width=0.9\linewidth]{Figure/qaoa-regular3.pdf}


    \includegraphics[width=0.9\linewidth]{Figure/qsim_rand_0.3.pdf}

    \includegraphics[width=0.9\linewidth]{Figure/qft.pdf}

    \includegraphics[width=0.9\linewidth]{Figure/vqe.pdf}

    \includegraphics[width=0.9\linewidth]{Figure/bv.pdf}

    \caption{Effects of the continuous routing algorithm and the introduction of zoned architecture on QAOA-regular3, QSIM-rand-0.3, QFT, VQE, and BV benchmark circuits. This study evaluates various numbers of qubits and focuses on four key components of overall circuit fidelity.}
    \label{fig:fidelity ablation}
\end{figure*}

% \paragraph{}
% Overall, our continuous routing and zoned architecture lead to notable improvements in both excitation and decoherence fidelity across different benchmark circuits.

% In this section, we evaluate the impact of continuous routing and zoned architecture on various components of fidelity as circuit scales increase across different benchmark circuits. 

% As shown in Fig. \ref{fig:fidelity ablation}(b)(e), for the QSIM-rand and BV cases, our fidelity demonstrates a much more noticeable improvement in excitation fidelity compared to the QAOA-regular3, QFT, and VQE cases with the zoned architecture, as shown in Fig. \ref{fig:fidelity ablation}(a)(c)(d). This is because that where are more single-qubit gates that do not commute with the CZ gate, resulting in a greater number of CZ blocks with dependency relationship and fewer CZ gates within each block. This leads to more Rydberg light execution stages and a reduced overall movement distance within each stage for the QSIM-rand and BV cases. This, in turn, results in a higher occurrence of excitation errors and less optimization space for decoherence fidelity, as shown in the blue and yellow part of Fig. \ref{fig:fidelity ablation}(b)(e). In contrast, the QAOA-regular3, QFT, and VQE cases feature fewer CZ blocks and more CZ interactions within each block, leading to reduced optimization space for excitation fidelity and increased space for decoherence fidelity, as shown in the blue and yellow part of Fig. \ref{fig:fidelity ablation}(a)(c)(d). Thus, our fidelity demonstrates a more significant improvement in decoherence fidelity with the continuous routing algorithm.
% \todo{lots of reference back... strange. Fig. 7 only shows in the third paragraph.}
% We also examine how execution time decreases with varying numbers of Application-Oriented Devices (AODs).


% As discussed in Section \ref{subsection: main results}, the continuous routing algorithm and the zoned architecture offer different levels of improvement in overall circuit fidelity. In this section, we thoroughly evaluate the performance of individual fidelity components across various benchmark circuits, analyzing how continuous routing and zoned architecture influence these components as the circuit scale increases.

% As mentioned in Section \ref{sec:conti router}, the continuous routing algorithm primarily aims to reduce both the number and distance of collective movements.  The number of collective movements is correlated with the number of transfers, which positively impacts transfer fidelity. Additionally, the overall movement distance directly impacts decoherence time, which in turn affects decoherence fidelity, as discussed in Section \ref{subsec:fidelity analysis}. Meanwhile, the zoned architecture, introduced in Section \ref{subsec: our motivation}, helps mitigate qubit excitation errors and can also improve decoherence fidelity. While the storage zone introduces additional inter-zone movements, potentially leading to more decoherence errors, the fact that qubits in the storage zone are negligibly affected by decoherence errors provides a compensatory benefit.





% In this section, we demonstrate that our framework supports significantly higher fidelity, enables parallel execution, and achieves shorter compilation time, highlighting its scalability for large-scale programs.

% \paragraph{Fidelity.}
% As shown in Fig. \ref{fig:fidelity ablation}, our framework significantly outperforms the Enola framework, which only achieves reasonable fidelity for small-scale programs. In contrast, our approach enables large-scale programs to maintain high fidelity, particularly in the QSIM-rand and BV cases. For instance, in the 70-qubit BV scenario, while Enola records a low fidelity of \(6.92 \times 10^{-4}\), our method sustains a fidelity of \(0.75\).

% \paragraph{Execution Time.}
% As discussed in Section \ref{sec:multi-AOD scheduler}, we can use multiple AODs to parallelize our collective moves. The execution time of compiled programs in our framework can be significantly reduced, as shown in Fig. \ref{fig:multi_aod}. Meanwhile, overall circuit fidelity remains stable or even   slightly improves, as the decrease in decoherence time with an increasing number of AODs leads to an enhancement in decoherence fidelity.

% \paragraph{Compilation Time.}
% Additionally, our framework demonstrates a significantly shorter compilation time compared to Enola, with improvements of up to 213.5 times, as shown in Table \ref{tab:runtime}. This enhancement remains stable or slightly increases as the program size expands. This reduction is primarily due to our near-linear heuristic algorithm for collective movement grouping, which enables a significant time reduction over the maximum independent set (MIS) solver used in Enola.


\begin{figure}[h!]
    \hspace{-30pt}
    \includegraphics[width=0.8\linewidth]{Figure/multi_aod.pdf}
    \caption{Effects of multiple AODs on the 100-qubit QAOA-regular3, 20-qubit QSIM-rand-0.3, 18-qubit QFT, 50-qubit VQE, and 70-qubit BV benchmark circuits.}

    \label{fig:multi_aod}
\end{figure}

% \begin{table}[h]
%     \centering
%       \caption{Compilation Time Comparison.}
%       % \vspace{-5pt}
      
%     \resizebox{0.48\textwidth}{!}{
%         \renewcommand*{\arraystretch}{1}
%         \begin{footnotesize}
%         \begin{tabular}{|p{2.4cm}|p{1.5cm}|p{1.6cm}|p{1.4cm}|}  \hline
%         Benchmark - \#Qubits & Enola Comp. Time ($s$) & Power Comp. Time ($s$) & Comp. Time Improv.\\ 
%         \hline
%         QAOA-regular4-20 & 251.68 & 63.42 & 3.97 \\
%         \hline
%         QAOA-regular4-50 & 253.94 & 63.34 & 4.01 \\
%         \hline
%         QAOA-regular4-80 & 291.68 & 72.17 & 4.04 \\
%         \hline
%         QAOA-rand-10 & 284.63 & 62.09 & 4.58 \\
%         \hline
%         QAOA-rand-30 & 1,791.66 & 193.28 & 9.27 \\
%         \hline
%         QAOA-rand-50 & 5,160.22 & 321.85 & 16.03 \\
%         \hline
%         QFT-18 & 10,917.79 & 347.47 & 31.42 \\
%         \hline
%         QFT-29 & 24,116.00 & 511.97 & 47.10 \\
%         \hline
%         QSIM-rand-10 & 760.19 & 76.01 & 10.00 \\
%         \hline
%         QSIM-rand-20 & 5,740.76 & 107.03 & 53.64 \\
%         \hline
%         QSIM-rand-40 & 8,283.45 & 127.95 & 64.74 \\
%         \hline
%         VQE-10 & 47.20 & 25.30 & 1.87 \\
%         \hline
%         VQE-30 & 57.62 & 29.68 & 1.94 \\
%         \hline
%         VQE-50 & 56.58 & 29.86 & 1.89 \\
%         \hline
%         BV-14 & 669.48 & 28.79 & 23.26 \\
%         \hline
%         BV-50 & 1,710.91 & 17.95 & 95.32 \\
%         \hline
%         BV-70 & 4,334.50 & 20.30 & 213.54 \\
%         \hline
         
%         \end{tabular}
%         \end{footnotesize}
%     }
%  % \vspace{-10pt}
%     \label{tab:runtime}
% \end{table}






==> TexFile/10_pseudo_code_rjx.tex <==

\begin{algorithm}
\caption{Schedule Interacting Movement}
\label{alg:pseudo_codes}
\footnotesize
% \fontsize{8.1pt}{9.6pt}\selectfont
\KwData{cur\_stage(current stage CZ interactions), pos(qubit positions)}
\KwResult{dir\_moves, undecided\_qubits, static\_qubits, pos}

\SetKwFunction{ScheduleMoveDirection}{ScheduleInteractMove}
\SetKwFunction{GetMoveInQubits}{GetMoveInQubits}
\SetKwFunction{GetMoveOutQubits}{GetMoveOutQubits}
\SetKwFunction{AssignDirectedMove}{AssignDirectedMove}
\SetKwFunction{GetUndecidedQubits}{GetUndecidedQubits}
\SetKwFunction{AssignUndecidedMove}{AssignUndecidedMove}
\SetKwFunction{AssignInStorageMove}{AssignInStorageMove}
\SetKwFunction{MoveUnify}{MoveUnify}

\SetKwProg{Fn}{Function}{:}{}
\Fn{\ScheduleMoveDirection{cur\_stage, pos}}{
    $in\_qubits, out\_qubits \leftarrow Empty\ list$;\\
    $undecided\_qubits \leftarrow Empty\ list$;\\
    $static\_qubits \leftarrow Empty\ map$;\\
    $dir\_moves \leftarrow Empty\ list$;\\
    
    \textit{\textbf{// identify the move-in and move-out storage qubits}}\\
    \If{$SF$}{
        $in\_qubits \leftarrow \GetMoveInQubits(s, pos)$;\\
        $out\_qubits \leftarrow \GetMoveOutQubits(s, pos)$;\\
    }
    
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\AssignDirectedMove{$q_0$, $q_1$, $undecided\_flag$}}{
        $dir\_moves.append((q_0, q_1))$;\\
        \If{$undecided\_flag$}{
            $undecided\_qubits.append(q_1)$;\\
        }
        \Else{
            $static\_qubits[pos[q_1]] \leftarrow q_1$;\\
        }
    }
    \textit{\textbf{// determine move/stay status for interacting qubits}}\\
    \For {$cz_i$ in $cur\_stage$}{
        $q_0, q_1 \leftarrow cz_i[0], cz_i[1]$;\\
        $pos\_q_0, pos\_q_1 \leftarrow pos[q_0], pos[q_1]$;\\
        \textit{\textbf{// $q_0$ and $q_1$ are both in storage zone}}\\
        \If {$q_0$ in $out\_qubits$ and $q_1$ in $out\_qubits$}{
            $\AssignDirectedMove(q_0, q_1, True)$;\\
            $continue$;\\
        }
        \If{$q_0$ in $out\_qubits$}{
            \textit{\textbf{// $pos\_q_1$ has not been assigned a static qubit}}\\
            \If {$pos\_q_1$ not in $static\_qubits.keys()$}{
                $\AssignDirectedMove(q_0, q_1, False)$;\\  
            }
            \Else{
                $\AssignDirectedMove(q_0, q_1, True)$;\\                     
            }
                $continue$;\\ 
        }
        \If{$q_1$ in $out\_qubits$}{
            \textit{\textbf{// $pos\_q_0$ has not been assigned a static qubit}}\\
            \If {$pos\_q_0$ not in $static\_qubits.keys()$}{
                $\AssignDirectedMove(q_1, q_0, False)$;\\  
            }
            \Else{
                $\AssignDirectedMove(q_1, q_0, True)$;\\                  
            }
                $continue$;\\ 
        }

        \If {$pos\_q_1$ not in $static\_qubits.keys()$}{
            $\AssignDirectedMove(q_0, q_1, False)$;\\
            $continue$;\\
        }
        
        \If {$pos\_q_0$ not in $static\_qubits.keys()$}{
            $\AssignDirectedMove(q_1, q_0, False)$;\\
            $continue$;\\
        }
        
        $\AssignDirectedMove(q_0, q_1, True)$;\\
    }
    $\Return \ dir\_moves, undecided\_qubits, static\_qubits, pos$;\\
}
\end{algorithm}


% \begin{algorithm}
% \caption{PowerMove}
% \label{alg:pseudo_codes}
% \footnotesize
% % \fontsize{8.1pt}{9.6pt}\selectfont
% % \KwData{G, DAG, D (\#delay lines), S (virtual layer size), lcount, Mem, $b_r$, $b_m$, CompleteNds, NdAllocLayer}
% % \KwResult{G, DAG, Mem, EG (embedded graph), IE (inter edges), lcount, m, CompleteNds, NdAllocLayer}
% \KwData{Circ(Quantum Cicuit), D(entanglement zone size = $D \times D$), SD(storage zone size = $D \times SD$), N(\#qubits), SF(storage flag)}
% \KwResult{R(compiled record)}

% \SetKwFunction{PowerMove}{PowerMove}
% \SetKwFunction{GetCZBlocks}{GetCZBlocks}
% \SetKwFunction{StageGenerator}{StageGenerator}
% \SetKwFunction{StageScheduler}{StageScheduler}
% \SetKwFunction{AtomPlacer}{AtomPlacer}
% \SetKwFunction{MoveDirScheduler}{MoveDirScheduler}
% \SetKwFunction{ColMoveGenerator}{ColMoveGenerator}
% \SetKwFunction{MoveScheduler}{MoveScheduler}
% \SetKwFunction{GetMoveInQubits}{GetMoveInQubits}
% \SetKwFunction{GetMoveOutQubits}{GetMoveOutQubits}
% \SetKwFunction{UnifyMoves}{UnifyMoves}
% \SetKwFunction{FSMoveGenerator}{FSMoveGenerator}
% \SetKwFunction{InMoveGenerator}{InMoveGenerator}
% \SetKwFunction{Update}{Update}
% \SetKwProg{Fn}{Function}{:}{}
% \Fn{\PowerMove{Circ, D, SD, N}}{
%     $blocks \leftarrow \GetCZBlocks(Circ, N)$;\\ 
%     $stages \leftarrow Empty\ list$;\\
%     \For{$b$ in $blocks$}{
%         $cur\_stages \leftarrow \StageGenerator(b, N)$;\\
%         \If{$SF$}{
%             $cur\_stages \leftarrow \StageScheduler(cur\_stages)$;\\
%         }
%         $stages \leftarrow stages + cur\_stages$;\\
%     }
%     $pos \leftarrow \AtomPlacer(N, stages, SF)$;\\
%     \For{$s$ in $stages$}{
%         $in\_qubits \leftarrow Empty\ list$;\\
%         $out\_qubits \leftarrow Empty\ list$;\\
%         \If{$SF$}{
%             $in\_qubits \leftarrow \GetMoveInQubits(s, pos)$;\\
%             $out\_qubits \leftarrow \GetMoveOutQubits(s, pos)$;\\
%         }
%         \textit{\textbf{// fs\_qubits refers to fake static qubits}}\\
%         $dir\_moves, fs\_qubits \leftarrow \MoveDirScheduler(s, out\_qubits, SF)$;\\
%         $fs\_moves \leftarrow \FSMoveGenerator(fs\_qubits, pos)$;\\
%         $in\_moves \leftarrow \InMoveGenerator(in\_qubits, pos)$;\\
%         $moves \leftarrow \UnifyMoves(dir\_moves, fs\_moves, in\_moves)$;\\
%         $col\_moves \leftarrow \ColMoveGenerator(moves)$;\\
%         \If{$SF$}{
%             $col\_moves \leftarrow \MoveScheduler(col\_moves, in\_qubits, out\_qubits)$;\\
%         }
%         $R, pos \leftarrow \Update(R, pos, col\_moves)$;\\
%     }
% }
% \end{algorithm}

